Near-Optimal Bayesian Online Assortment of Reusable Resources

Motivated by the applications of rental services in e-commerce, we consider revenue maximization in online assortment of reusable resources for a stream of arriving consumers with different types. We design competitive online algorithms with respect to the optimum online policy in the Bayesian setting, in which types are drawn independently from known heterogeneous distributions over time. In the regime where the minimum of initial inventories $c_0$ is large, our main result is a near-optimal $1-\min\left(\frac{1}{2},\sqrt{\log(c_0)/c_0}\right)$ competitive algorithm for the general case of reusable resources. Our algorithm relies on an expected LP benchmark for the problem, solves this LP, and simulates the solution through an independent randomized rounding. The main challenge is obtaining point-wise inventory feasibility in a computationally efficient fashion from these simulation-based algorithms. To this end, we use several technical ingredients to design $\textit{discarding policies}$ -- one for each resource. These policies handle the trade-off between the inventory feasibility under reusability and the revenue loss of each of the resources. However, discarding a unit of a resource changes the future consumption of other resources. To handle this new challenge, we also introduce $\textit{post-processing}$ assortment procedures that help with designing and analyzing our discarding policies as they run in parallel, which might be of independent interest. As a side result, by leveraging techniques from the literature on prophet inequality, we further show an improved near-optimal $1-1/\sqrt{c_0+3}$ competitive algorithm for the special case of non-reusable resources. We finally evaluate the performance of our algorithms using the numerical simulations on the synthetic data.

==> tex/acknowledgement.tex <==
We are grateful to Vineet Goyal, Garud Iyengar, and Rajan Udwani for pointing us to an error in an earlier version of this manuscript. 

==> tex/adversarial-general.tex <==
\label{app:general-penalty}
In this section,
we prove \Cref{prop:concave competitive ratio-iid}. As a corollary, this will also prove \Cref{thm:concave competitive ratio}, simply because the reverse and forward expected LP are equivalent programs when rental times are fixed over time (\Cref{remark:iid-fixed}). This result
extends the result of \citet{GNR-14}
for arbitrary concave penalty functions
from infinite rental time setting
to our setting (i.e., i.i.d.\ stochastic rental times), but the competitive ratio is measured against the optimal objective value of the reverse expected LP.
To this end, we follow a similar randomized primal-dual argument 
as in \Cref{thm:exponential competitive ratio} 
but with a more involved 
algorithmically constructed dual solution.
Specifically, we introduce a sub-problem termed as \emph{Interval Assignment Problem (IAP)},
and an algorithm to solve it. We use the solution produced by this algorithm as a guide 
to construct the dual solution. 

\begin{definition}[Interval Assignment Problem (IAP)]
\label{def:IAP}
Consider $n$ intervals $\{[a_1, b_1], \dots, [a_n, b_n]\}$ 
defined on $\R$, where 
interval $i$ is from $a_i$ to $b_i$
and 
$a_1 < a_2 < \dots < a_n$.
Let $\contain_i$ be a subset of $n$ intervals
which covers position $a_i$,
i.e., $\contain_i = \{j\in[n]: a_i \in [a_j, b_j]\}$
and $\containn_i$ be its size, i.e., $\containn_i = |\contain_i|$.
\emph{Interval Assignment Problem}
requires to construct
an assignment $\{\assign_1, \dots, \assign_n\}\in\mathbb{Z}_{\geq 0}^n$ 
for our intervals that satisfies the following three properties,
\begin{itemize}
\item \textbf{Local Dominance:}
For each interval $i \in [n]$,
there exists a bijection $\rho_i:\contain_i \rightarrow \{1, 2, \dots, \containn_i\}$
such that for all $j \in \contain_i$, $\assign_j \geq \rho_i(j)$.

\item \textbf{Global Dominance:}
For any decreasing and concave function $\bar\pen$,
$\sum_{i\in[n]} \bar\pen(\assign_i) \geq \sum_{i \in [n]} \bar\pen(\containn_i)$.
%the number of interval $i$ with $\containn_i \geq c$
%is at least 
%the number of interval $i$ with $\assign_i \geq c$,
%i.e.,
%$
%|\{i\in[n]:\containn_i \geq c\}| \geq 
%|\{i\in[n]:\assign_i \geq c\}|
%$.

\item \textbf{Partition Monotonicity:}
$n$ intervals can be partition into $m$ subgroups $A_1, A_2, \dots, A_m$
for some integer $m$ such that 
for all $k \in [m]$,
$
\{\assign_i: i \in A_k\} 
= 
\{
1, 2, \dots, |A_k|
\}
$.
\end{itemize}
\end{definition}

\begin{algorithm}[t]
\caption{Interval Assignment Solver
}\label{alg:interval assignment}
\begin{algorithmic}[1]

\State Initialize an assignment vector
$\assign_i = 0$ for all $i \in [n]$.
\State Initialize a pointer vector 
$\pfather_i = -1$ for all $i \in [n]$. 

\State Initialize a pointer vector
$\pmother_i = -1$  for all $i \in [n]$.

\State Initialize the remaining interval set 
$\remaining = \{1, 2, \dots, n\}$,
define $\remainingcontain_i = \contain_i \cap \remaining$
and $\remainingcontainn_i = |\remainingcontain_i|$.
%and $\remainingcontainn_i = |\contain_i \cap \remaining|$.

\While{$\remaining$ is not empty}
\State \begin{varwidth}[t]{\linewidth}
Find the interval $i$ with the largest index 
in the remaining interval set $\remaining$
%	  \par
%\hskip\algorithmicindent  
where $\remainingcontainn_i$ is maximized, 
i.e., $i =\,%\{
\argmax_{i\in W} \{\remainingcontainn_i
%\}
\}$. 
%\par\hskip
\end{varwidth}
\vspace{+1mm}
\State \begin{varwidth}[t]{\linewidth}
Find the interval $j$ with the smallest index %left most starting point
in the remaining interval set $\remaining$
which
covers position $a_i$,
i.e., $j = \min \remainingcontain_i$.
\end{varwidth}
\vspace{+1mm}
\State Set $\assign_j = \remainingcontainn_i$ and $\pmother_j = i$.

\For{all $k \in [n] / \remaining$ such that 
$j \in \contain_{\pmother_k}$ and $\assign_k = \assign_j + 1$}
\State Set $\pfather_k = j$. 
\EndFor

\State  
%\begin{varwidth}[t]{\linewidth}
Remove interval $j$ from the remaining interval set $\remaining$ %, and update $C(t)$ 
%for all remaining interval $t$,\par
%\hskip\algorithmicindent  
i.e., set
$\remaining = \remaining / \{j\}$.
%$C(t) = \{\tpre \in R \given 
%\tpre \leq t, f(\tpre) \geq t\}$.
%\end{varwidth}
\EndWhile
\State Return $\{\assign_1, \dots, \assign_n\}$.
\end{algorithmic}
\end{algorithm}

\begin{lemma}
For any input instance,
the solution of Interval Assignment Problem exists. Specifically, 
\Cref{alg:interval assignment} outputs such a solution.
\end{lemma}

\begin{proof}
In each iteration, \Cref{alg:interval assignment} 
pins down the assignment for a remaining interval and then remove it.
Thus, the algorithm terminates and outputs an assignment $\{\assign_1, \dots, \assign_n\}$.
We next show this assignment satisfies \emph{Local Dominance}, \emph{Global Dominance}
and \emph{Partition Monotonicity} separately.

\noindent\emph{\rom{1}. Local Dominance.}
%\paragraph{Local Dominance} 
For each interval $i \in [n]$,
consider $j_1, j_2, \dots \in \contain_i$ in the order which they are
removed from the algorithm:
for the $k$-th removed interval $j_k \in \contain_i$,
at that time $\remainingcontainn_i$ is $\containn_i - k + 1$,
which guarantees that $\assign_{j_k}$ is at least $\containn_i - k + 1$.
Thus, \emph{Local Dominance} is satisfied.


\noindent\emph{\rom{2}. Global Dominance.}
%\paragraph{Global Dominance}
We prove this by induction. Consider the reverse order of intervals removed
from the remaining interval set $\remaining$ in the algorithm,
i.e., we set $\remaining = \emptyset$ as the base case and then add intervals back to $\remaining$
in the reverse order which they have been removed in the algorithm. 
Our induction hypothesis is that restrict to intervals in $\remaining$,
\emph{Global Dominance} holds,
i.e., for any decreasing and concave function $\bar\pen$,
\begin{align}
\label{eq:global dominance}
\sum_{i\in \remaining} \bar\pen(\assign_i) \geq \sum_{i \in \remaining} \bar\pen(\remainingcontainn_i).
\end{align}

\emph{Base Case ($\remaining = \emptyset$):} In this case, the induction hypothesis holds trivially.

\emph{Inductive Step:}  Suppose the induction hypothesis holds before we add interval $i$ 
with $\assign_{i}$ back
to $\remaining$. 
Let $m = \assign_{i} - 1$.
To make it clear, let $\remaining$ to be the remaining interval set before we add interval $i$,
and $\remaining'$ to be the remaining interval set after we add interval $i$, i.e., 
$\remaining' = \remaining \cup\{i\}$.
%Let $\assign^{-1}(c) = |\{j \in W: \assign_j = c\}|$
%and 
%$\containn^{-1}(c) = |\{j \in W: |\contain_j \cap W| = c\}|$.
Next we consider the increment of both sides in 
\eqref{eq:global dominance}
after 
we add interval $i$ into $\remaining$.
The left hand side of \eqref{eq:global dominance} increases by $\bar\pen(m + 1)$.
%$\assign^{-1}(k)$ increases by one 
%while $\assign^{-1}(k')$ does not change for all $k' \not=k$.
For the right side, since $\assign_i = m + 1$,
there exist $m$ intervals $j_1, j_2, \dots j_m \in \remaining$
which 
%such that interval $j_k$ 
cover position $a_{\pmother_i}$,
and $i < j_k$ (otherwise, $j_k$ should be removed early than $i$ in the algorithm)
for all $k\in[m]$.
This implies that interval $i$ covers position $a_{j_k}$ 
for all $k \in[m]$.
Without loss of generality, we assume $j_1 < j_2 < \dots < j_m$,
then $\remainingcontainn_{j_k} \geq k$.
Hence, once we add interval $i$ into $W$,
the right hand side of \eqref{eq:global dominance}
increases by 
\begin{align*} &
\bar\pen(\containn_i^{\remaining'}) + 
\sum_{j\in \remaining}
\left(
\bar\pen(\containn_{j}^{\remaining'}) - 
\bar\pen(\remainingcontainn_{j})
\right) \\
\leq&\bar\pen(\containn_i^{\remaining'}) + 
\sum_{k\in[m]}
\left(
\bar\pen(\containn_{j_k}^{\remaining'}) - 
\bar\pen(\remainingcontainn_{j_k})
\right) \\
=&
\bar\pen(\containn_i^{\remaining'}) + 
\sum_{k\in[m]}
(\bar\pen(\remainingcontainn_{j_k} + 1) - 
\bar\pen(\remainingcontainn_{j_k})) \\ 
\overset{(a)}{\leq} &
\bar\pen(1) + 
\sum_{k \in [m]}
(
\bar\pen(k + 1) - \bar\pen(k)
) 
= \bar\pen(m + 1)
\end{align*}
where (a) holds because $\bar\pen$ is decreasing and concave.
Applying the induction hypothesis (before we add interval $i$),
the induction hypothesis (after we add interval $i$) holds,
which finishes the induction.

\noindent\emph{\rom{3}. Partition Monotonicity.}
%\paragraph{Partition Monotonicity}
We first introduce the following two claims:
(a) for each interval $i\in[n]$, there is at most one interval $j$ such that
$\pfather_j = i$;
(b) for each interval $i\in[n]$ with $\assign_i > 1$, $\pfather_i \not= -1$.  
Notice that claim (a) and (b) together imply that $\{\pfather_1, \dots, \pfather_n\}$ 
defines a partition which satisfies \emph{Partition Monotonicity} as follows:
\begin{enumerate}
\item[(i)] find an interval $i$ 
which is not in any current subgroups
and $\pfather_j \not= i$ for all $j\in[n]$
(halt if such interval $i$ does not exist)
\item[(ii)] create a new subgroup $A$,
\item[(iii)] while $\pfather_i \not= -1$, add interval $i$ into $A$, set $i = \pfather_i$, while end.
\item[(iv)] back to step (i).
\end{enumerate}
Next, we show claim (a) and claim (b) separately.

We show claim (a) by contradiction. 
Suppose there exists interval $i$, $j_1$ and $j_2$ such that 
$\pfather_{j_1} = \pfather_{j_2} = i$.
By the construction of the algorithm,
$\assign_{j_1} = \assign_{j_2} = \assign_i + 1$.
Now, consider case by case.
\begin{itemize}
\item \emph{Case 1 ($i < j_1$ or $i < j_2$):} Without loss of generality, we assume $i < j_1$,
and the case $i < j_2$ is symmetric.
%Consider the moment when the algorithm 
%removes interval $j_1$ due to $\pmother_{j_1}$.
By the construction of the algorithm,
$\pfather_{j_1} = i$ implies 
$i \in \contain_{\pmother_{j_1}}$. 
%interavl $i$ also covers position $a_{\pmother_{j_1}}$,
This leads to a contradiction, because 
if $i < j_1$, interval $i$ should be removed early than interval $j_1$ in the algorithm 
which implies $\assign_i \geq \assign_{j_1}$.
\item \emph{Case2 ($j_1, j_2 < i$):}
\begin{itemize}
\item \emph{Case 2a ($\pmother_{j_1} < \pmother_{j_2}$ or $\pmother_{j_2} < \pmother_{j_1}$):}
Without loss of generality, we assume $\pmother_{j_1} < \pmother_{j_2}$
and the case $\pmother_{j_2} < \pmother_{j_1}$ is symmetric.
\begin{itemize}
\item \emph{Case 2a1 (interval $j_1$ is removed before interval $j_2$):}
In this case, consider the moment 
when the algorithm removes $j_1$ due to interval $\pmother_{j_1}$.
By the construction of the algorithm, since $j_1$ is removed before $j_2$,
it implies
$\remainingcontainn_{\pmother_{j_1}} > \remainingcontainn_{\pmother_{j_2}}$.
Thus,
$\assign_{j_1}$ is strictly larger than $\assign_{j_2}$,
contradiction.
\item \emph{Case 2a2 (interval $j_2$ is removed before interval $j_1$):}
In this case, consider the moment 
when the algorithm remove $j_2$ due to interval $\pmother_{j_2}$.
Notice that interval $j_2$ also covers position $a_{\pmother_{j_1}}$,
i.e., $j_2 \in \contain_{\pmother_{j_1}}$.
By the construction of the algorithm, since $j_2$ is removed before $j_1$,
it implies
$\remainingcontainn_{\pmother_{j_1}}  \leq \remainingcontainn_{\pmother_{j_2}}$.
Thus, once the algorithm removed $j_2$, 
$\containn_{\pmother_{j_1}}^{\remaining/\{j_2\}}$ (which is an upper bound
of $\assign_{j_1}$) 
becomes strictly smaller than 
$\remainingcontainn_{\pmother_{j_2}}$ (which is equal to $\assign_{j_2}$), %which 
%implies $\assign_{j_1}$ is strictly smaller than $\assign_{j_2}$,
contradiction.
\end{itemize}

\item \emph{Case 2b ($\pmother_{j_1} = \pmother_{j_2}$):}
Without loss of generality, we assume interval $j_1$ is removed before interval $j_2$,
and the case where interval $j_2$ is removed before interval $j_1$ is 
symmetric.
Let $\pmother^* = \pmother_{j_1} = \pmother_{j_2}$. Consider the moment
when the algorithm removes $j_1$ due to $\pmother^*$.
By the construction of the algorithm,
$\assign_{j_1} = \remainingcontainn_{\pmother^*}$
and $\assign_{j_2} \leq \containn_{\pmother^*}^{\remaining/\{j_1\}} 
= \remainingcontainn_{\pmother^*} - 1$.
Thus, $\assign_{j_1}$ is strictly larger than $\assign_{j_2}$,
contradiction.
\end{itemize}
\end{itemize}

We show claim (b) as follows. For any interval $i$
with $\assign_i > 1$,
consider the next removed interval $j$ %which covers 
%position $a_{q_i}$ and is the first interval removed 
among
$\contain_{\pmother_i}$ after the algorithm removes interval $i$.
It is sufficient to show $\assign_j = \assign_i - 1$,
which implies that algorithm set $\pfather_i = j$ when it removes interval $j$.
Since $j$ is the next interval removed among $\contain_{\pmother_i}$ after 
interval $i$, $\assign_i - 1\leq \assign_j \leq \assign_i$.
To show $\assign_j < \assign_i$, we use contradiction.
Suppose $\assign_j = \assign_i$. If $i\in\contain_{\pmother_j}$,
this implies that at the moment when the algorithm removes $i$, 
$
\assign_i = \containn_{\pmother_i}^{\remaining}
\geq
\containn_{\pmother_j}^{\remaining} \geq \assign_j + 1 = \assign_i + 1
$, contradiction.
If $i \not\in \contain_{\pmother_j}$, since $i < j$, 
it implies that $\pmother_i < \pmother_j$ and
at the moment when the algorithm removes $i$,
$\containn_{\pmother_i}^\remaining
=
\assign_i
=\assign_j 
\leq \containn_{\pmother_j}^\remaining
$, contradiction.
\qedhere
\end{proof}

We present the formal proof of \Cref{thm:concave competitive ratio} below.

\begin{proof}[Proof of \Cref{prop:concave competitive ratio-iid}]
We start with the offline expected LP on the reverse type sequence, i.e., $\EAR{\inversetypesequence}$
where $\type_t' = \type_{\totaltime - t + 1}$,
\begin{align*}
%\nonumber
&\begin{array}{rlll}
\max
\limits_{\mathbf \alloc \geq \mathbf 0} &
\displaystyle\sum\nolimits%\limits
_{t=1}^\totaltime
\displaystyle\sum\nolimits%\limits
_{\assortment \in \assortmentspace}
\displaystyle\sum\nolimits%\limits
_{i=1}^n
\reward_i\curchoice\curalloc
&
\text{s.t.}
&\\ %& & &\\
&
\displaystyle\sum\nolimits_{\tpre = t}^{\totaltime}
\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
%(1-\durationdistribution_i(t - \tpre)) 
%\prob[\durationdistribution_i]{\duration_{i,\tpre} \geq \tpre - t}
\durationcdfi_i(\tpre - t)
\prechoice\prealloc \leq \inventory_i
& i \in [n],\ t \in [\totaltime]
%\forall i\in[n],t \in [T] 
&\langle\inventorydual\rangle
\\
&\displaystyle\sum\nolimits_{\assortment\in \assortmentspace}\curalloc \leq 1
&t \in [\totaltime]
&\langle\probdual\rangle \\
%\end{array}\\
\intertext{We construct its dual program with dual variable $\inventorydual$ 
and $\probdual$ as follows,} 
%\nonumber
%	&\begin{array}{rlll}
\min
\limits_{\boldsymbol{\theta},\boldsymbol{\lambda} \geq \mathbf 0} &
\displaystyle\sum\nolimits%\limits
_{t=1}^\totaltime
\displaystyle\sum\nolimits%\limits
_{i=1}^n
\inventory_i\inventorydual
+
\displaystyle\sum\nolimits_{t =1}^\totaltime
\probdual
& 
\text{s.t.} 
&\\ %& & &\\
&
\probdual + 
\displaystyle\sum\nolimits_{i = 1}^n
\displaystyle\sum\nolimits_{\tpre= 1}^t
%(1-\durationdistribution_i(t - \tpre)) 
%\prob[\durationdistribution_i]{\duration_{i,\tpre} \geq t - \tpre}
\durationcdfi_i(t - \tpre)
\curchoice\theta_{i,\tpre}
%& & \\
%				&  
%		\qquad\qquad
%		\qquad\qquad
%		\qquad\qquad
%		\qquad\qquad
\geq \displaystyle\sum\nolimits_{i = 1}^n
\reward_i\curchoice
& \assortment \in \assortmentspace,\ t \in [\totaltime]
%\forall i\in[n],t \in [T] 
&\langle\curalloc\rangle
\end{array}
\end{align*}	
Let $\assortment_t$ be the assortment offered to consumer $t$.
Recall $\curinventorya$ 
%(resp.\ $\curinventoryb$) 
is the 
inventory level of product $i$ at time period $t$ 
before 
%(resp.\ after) 
the realization of 
consumer selection. 
For each product $i$,
consider the following 
instance of the Interval Assignment Problem (IAP)
in \Cref{def:IAP}
separately.
Let 
%it has been allocated at time 
$\texttt{alloc}_i = \{t_1, t_2, \dots, t_m\}$
be the time periods when product $i$ is selected,
and let 
the correpsonding rental duration of product $i$ be 
$d_{t_1}, d_{t_2}, \dots, d_{t_m}$, respectively.
Let the instance of IAP with $m$ intervals,
where each interval $[t_j, t_j + d_{t_j}]$ corresponds to 
the event that a unit of product $i$ has been selected 
by a consumer at time $t_j$ and returned to the platform 
at time $t_j + d_{t_j}$.
Let 
$\{\assign_{i, t}\}_{t\in \texttt{alloc}_i}$ 
be the assignment solved in IAP for product $i$ 
and let 
$\pseudoinventory_{i, t} = \inventory_i - \assign_{i, t}$ if $t \in \texttt{alloc}_i$
and $\pseudoinventory_{i, t} = 1$ otherwise.
Consider the following assignments for primal 
of (forward) expected LP, 
and dual 
of the reverse expected LP,
\begin{align*}
\textit{Primal:}~~~~~\curalloc &= \indicator{\assortment_t = \assortment},\\
\textit{Dual:}~~~~~~~ \probdual &= \displaystyle\sum\nolimits_{i = 1}^n \reward_i 
\pen\left(\frac{\curinventorya}{\inventory_i}\right)
\cdot
\indicator{\text{product $i$ is selected at time $t$}},\\
~~~~~~~~\inventorydual &= \reward_i\left(
\pen\left(\frac{\curpseudoinventory}{\inventory_i}\right) -
\pen\left(\frac{\curpseudoinventory - 1}{\inventory_i}\right)
\right) 
\cdot
\indicator{\text{product $i$ is selected at time $t$}}
\end{align*}
where 
$\indicator{\cdot}$ is an indicator operator. Note that product $i$ is selected at time $t$ if it belongs to the assortment set $\assortment_t$ and consumer arriving at time $t$ chooses this product.  In the rest of analysis, we show that the above primal assignment is feasible in the primal of forward expected LP, the above randomized dual assignment is feasible in expectation in the dual of reverse  expected LP, and finally the expected objective value of primal is at least $\alpha= \GNRnotation$ fraction of the expected objective value of the dual. Similar to  \Cref{lem:random primal-dual}, satisfying these properties is enough to finish the proof.
\vspace{1mm}

%Construct 
%the following solution of primal and dual,
%\begin{align*}
%	\curalloc &= 
%	\indicator{\assortment_t = \assortment},
%\left\{
%\begin{array}{ll}
%	1 \qquad & \text{if } \assortment = \assortment_t \\
%	0 & \text{otherwise.}
%\end{array}
%\right. 
%\;\;\;
%\;\;\;
%\qquad\qquad
%\qquad\qquad
%\qquad\quad
%	\probdual 
%	= 
%\displaystyle\sum\nolimits_{i = 1}^n \reward_i \choice^{\type_t}(\assortment_t, i)\curpena
%	\displaystyle\sum\nolimits_{i = 1}^n \reward_i 
%	\pen\left(\frac{\curinventorya}{\inventory_i}\right)
%	\cdot
%	\indicator{\text{product $i$ is selected at time $t$}},
%	\\ %\mbox{and}\;\;
%	\inventorydual &= \reward_i\left(
%	\pen\left(\frac{\curpseudoinventory}{\inventory_i}\right) -
%	\pen\left(\frac{\curpseudoinventory - 1}{\inventory_i}\right)
%\right) 
%\cdot
%\indicator{\text{product $i$ is selected at time $t$}}
%																								\end{align*}
%where 
%$\indicator{\text{product $i$ is selected at time $t$}}$ is the indicator
%variable that consumer selects product $i$ at time $t$,
%and 
%$\indicator{\assortment_t = \assortment}$
%is the indicator variable that assortment $\assortment$ is offered at time $t$.

%\paragraph{Feasibility of primal solution}
%Due to the property of Inventory-Balancing, i.e., $S_t$ offered by IB is always
%inventory feasible, the primal solution is feasible.

\noindent\emph{\rom{1}. Primal feasibility and dual feasibility in expectation.}
The primal assignment is feasible, 
as Inventory-Balancing only offers inventory feasible assortments. 
To show dual feasibility in expectation, 
first note that $\pen(.)$ is non-negative and monotone non-decreasing. 
Therefore $\probdual\geq 0$ for all $t\in[\totaltime]$, 
and $\inventorydual\geq 0$ for all $i\in[n],t\in[\totaltime]$. 
Next, we show for every $t\in[\totaltime]$ and $\assortment\in\assortmentspace$, 
the dual assignment satisfies the dual constraints 
corresponding to $\curalloc$ in expectation. 
Let $\indicator{\duration_{i,\tpre} \geq t - \tpre}$ be the indicator 
of the event that rental time of product $i$ at time $\tpre$ is at least 
$t - \tpre$. For every product $i\in[n]$, the following inequality holds at every time $t\in[\totaltime]$: 
%
%\paragraph{Feasibility of expected dual solution}
%To see that the dual solution is feasible in expectation, 
%let $\indicator{\duration_{i,\tpre} \geq t - \tpre}$ be the indicator variable 
%that the rental duration of product $i$ at time $\tpre$ is at least 
%$t - \tpre$.
%We first show that the following inequality holds for all product $i$, 
%all time $t$ and all realization,
\begin{align}
\label{eq:dual feasible ex post concave}
\reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right) 
+ \displaystyle\sum\nolimits_{\tpre = 1}^{t - 1}
\indicator{\duration_{i,\tpre} \geq t - \tpre} \cdot
\theta_{i, \tpre} 
\geq \reward_i
\end{align}
To see why inequality~\eqref{eq:dual feasible ex post concave} holds, 
consider on-hand units and under rental units of product $i$ at time $t$. 
Since the inventory level of product $i$ at time $t$  is 
$\curinventorya$, 
there are $\inventory_i - \curinventorya$ units of product $i$ 
under rental at that moment. Suppose these units were rented at times
$\tpre_1, \tpre_2, \dots, \tpre_{\inventory_i - \curinventorya}$,
where $\indicator{d_{\tpre_j} \geq t - \tpre_j} = 1$ and 
$\indicator{\text{product $i$ is selected at time $\tpre_j$}} = 1$
for all $j\in[\inventory_i - \curinventorya]$.
Additionally, recall 
$\{\assign_{i, t}\}_{t\in \texttt{alloc}_i}$ is assignment in IAP which satisfies
\emph{Local Dominance}.
%Consider interval start at 
%$\tpre_{\inventory_i - \curinventorya}$.
%$[\tpre_{\inventory_i - \curinventorya}, \tpre_{\inventory_i - \curinventorya} + 
%\duration_{i,\tpre_{\inventory_i - \curinventorya}}]$.
By Local Dominance at interval starting at $\tpre_{\inventory_i - \curinventorya}$,
there exists a bijection $\rho$ from $\contain_{\tpre_{\inventory_i - \curinventorya}}$
to $\{1,2,\dots,\containn_{\tpre_{\inventory_i - \curinventorya}}\}$ such that 
$\assign_{\tpre} \geq \rho(\tpre)$ for all $\tpre \in \contain_{\tpre_{\inventory_i - \curinventorya}}$.
Notice that intervals starting at 
$\tpre_1, \tpre_2, \dots \tpre_{\inventory_i - \curinventorya}$
all cover time $\tpre_{\inventory_i - \curinventorya}$,
i.e.,
$\tpre_j \in \contain_{\tpre_{\inventory_i - \curinventorya}}$ for all 
$j\in[\inventory_i - \curinventorya]$.
This implies there exists another bijection $\rho'$ from
$[\inventory_i - \curinventorya]$
to $[\inventory_i - \curinventorya]$
such that
$\assign_{\tpre_j} \geq \rho'(j)$
for all $j \in [\inventory_i - \curinventorya]$.
Because the penalty function $\pen(\cdot)$ is concave and increasing,
\begin{align}
\begin{split}
\label{eq:concave concave}
\theta_{i, \tpre_j} &= 
\reward_i\left(\pen\left(\frac{\pseudoinventory_{i, \tpre_j}}{\inventory_i}\right)
-
\pen\left(\frac{\pseudoinventory_{i, \tpre_j} - 1}{\inventory_i}\right)\right)  \\
&=
\reward_i\left(\pen\left(\frac{\inventory_i - \assign_{i, \tpre_j}}{\inventory_i}\right)
-
\pen\left(\frac{\inventory_i - \assign_{i, \tpre_j} - 1}{\inventory_i}\right)\right)  \\
&\geq
\reward_i\left(\pen\left(\frac{\inventory_i - \rho'(j)}{\inventory_i}\right)
-
\pen\left(\frac{\inventory_i - \rho'(j) - 1}{\inventory_i}\right)\right)
\end{split}
\end{align}
By applying \eqref{eq:concave concave}, 
we can prove inequality~\eqref{eq:dual feasible ex post concave}:
\begin{align*}
&\quad~\reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right) 
+ \displaystyle\sum\nolimits_{\tpre = 1}^{t - 1}
\indicator{\duration_{i, \tpre} \geq t - \tpre} \cdot
\theta_{i, \tpre}\\
& =\reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right) 
+ \displaystyle\sum\nolimits_{j = 1}^{\inventory_i - \curinventorya} \reward_i
\left(\pen\left(\frac{\pseudoinventory_{i, \tpre_j}}{\inventory_i}\right)
-
\pen\left(\frac{\pseudoinventory_{i, \tpre_j} - 1}{\inventory_i}\right)\right)\\
&\geq \reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right) + \displaystyle\sum\nolimits_{j = 1}^{\inventory_i - \curinventorya} \reward_i\left(\pen\left(\frac{\inventory_i - \rho'(j)}{\inventory_i}\right)
-
\pen\left(\frac{\inventory_i - \rho'(j) - 1}{\inventory_i}\right)\right)\\
&=\reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right) +\displaystyle\sum\nolimits_{I = \curinventoryb}^{\inventory_i - 1} 
\reward_i\left(
\pen\left(\frac{I}{\inventory_i}\right) 
-
\pen\left(\frac{I-1}{\inventory_i}\right) 
\right)\\
&=
\pen\left(\frac{\inventory_i - 1}{\inventory_i}\right) 
+
\pen\left(\frac{\curinventorya}{\inventory_i}\right) 
-
\pen\left(\frac{\curinventorya-1}{\inventory_i}\right) 
\geq\reward_i\pen(1)=\reward_i
\end{align*}

Now, for each time $t\in[\totaltime]$ and assortment $\assortment\in\assortmentspace$, consider the following expression:
\begin{align}
\label{eq:dual LHS concave}
\probdual + 
\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = 1}^t
\indicator{\duration_{i, \tpre} \geq t - \tpre}
\curchoice \theta_{i, \tpre} 
\end{align}
On the one hand, note that by taking expectation from \eqref{eq:dual LHS concave} we have 
\begin{equation}
\label{eq:first-compare concave}
\expect{\probdual + 
\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = 1}^t
\indicator{\duration_{i, \tpre} \geq t - \tpre}
\curchoice \theta_{i, \tpre} }=\expect{\probdual} + 
\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = 1}^t
\durationcdfi_i(t - \tpre)
\curchoice\expect{ \theta_{i, \tpre}}~,
\end{equation}
simply because $\theta_{i, \tpre}$ and $\indicator{\duration_{i, \tpre} \geq t - \tpre}$ are independent random variables (as rental time $\duration_{i, \tpre}$ is realized independently from the assortment and the consumer's selection at any time $\tpre$). On the other hand, by taking expectation from 
\eqref{eq:dual LHS concave} first over the randomness in the choice of consumer at time $t$, i.e., by conditioning on (i) history up to time $t$ (including rental times $\{\duration_{i, \tpre}\}_{\tpre=1}^{t-1}$ and the inventory levels $\curinventorya$ for each product $i$), and (ii) assortment $\assortment_t$ offered at time $t$, we have
%(notice that this is independent of all events before $t$ or 
%the assortment $\assortment_t$ offered at time $t$ or 
%the inventory level at time $t$),
\begin{align}
&\expect{\probdual + 
\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = 1}^t
\indicator{\duration_{i, \tpre} \geq t - \tpre}
\curchoice \theta_{i, \tpre} |\mathcal{F}_{t-1},\assortment_t}\nonumber\\
=&\displaystyle\sum\nolimits_{i = 1}^n 
\reward_i\choice^{\type_t}(\assortment_t, i)
\pen\left(\frac{\curinventorya}{\inventory_i}\right)
+	
\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = 1}^{t - 1}
\indicator{\duration_{i, \tpre} \geq t - \tpre}
\curchoice \theta_{i, \tpre} \nonumber \\
&+
\displaystyle\sum\nolimits_{i = 1}^n 
\choice^{\type_t}(\assortment, i)\reward_i
\choice^{\type_t}(\assortment_t, i)
\left(
\pen\left(\frac{\curpseudoinventory}{\inventory_i}\right)
-
\pen\left(\frac{\curpseudoinventory - 1}{\inventory_i}\right)
\right)\label{eq:third-term concave}\\
\overset{(a)}{\geq} &
\displaystyle\sum\nolimits_{i = 1}^n 
\reward_i\curchoice
\pen\left(\frac{\curinventorya}{\inventory_i}\right)
+	
\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = 1}^{t - 1}
\indicator{\duration_{i, \tpre} \geq t - \tpre}
\curchoice \theta_{i, \tpre}\nonumber  \\
=&\displaystyle\sum\nolimits_{i = 1}^n 
\curchoice\left(\reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right)+ \displaystyle\sum\nolimits_{\tpre = 1}^{t - 1}
\indicator{\duration_{i, \tpre} \geq t - \tpre} \cdot
\theta_{i, \tpre}  \right)
\nonumber \\
\overset{(b)}{\geq}& \displaystyle\sum\nolimits_{i = 1}^n 
\reward_i\curchoice~,\nonumber
\end{align}
where $\mathcal{F}_{t-1}$ denotes the history up to time $t$. Note that inequality~(a) above holds because $$
\assortment_t = 
\argmax_{\assortment \in \assortmentspace}\displaystyle\sum\nolimits_{i = 1}^n\reward_i\curchoice
\pen\left(\frac{\curinventorya}{\inventory_i}\right)~,
$$
and the third term in expression~\eqref{eq:third-term concave} is non-negative, and inequality~(b) holds because of  inequality~\eqref{eq:dual feasible ex post concave}. Therefore, by taking full expectation we have
\begin{equation}
\label{eq:second-compare concave}
\expect{\probdual + 
\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = 1}^t
\indicator{\duration_{i, \tpre} \geq t - \tpre}
\curchoice \theta_{i, \tpre} }\geq \displaystyle\sum\nolimits_{i = 1}^n 
\reward_i\curchoice
\end{equation}
Combining \eqref{eq:first-compare concave} and \eqref{eq:second-compare concave} shows feasibility in expectation of the dual assignment.
%	\begin{align}
%		\label{eq:dual feasible ex post final}
%		\eqref{eq:feasibility ex post} 
%		\geq 
%		\displaystyle\sum\nolimits_{i = 1}^n 
%		\reward_i\curchoice
%		\pen\left(\frac{\curinventorya}{\inventory_i}\right)
%		&+	
%		\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = 1}^{t - 1}
%		\indicator{\duration_{i, \tpre} \geq t - \tpre}
%		\curchoice \theta_{i, \tpre}  
%	\end{align}
%	Applying inequality \eqref{eq:dual feasible ex post}, it implies
%	\begin{align*}
%		\eqref{eq:feasibility ex post} 
%		\geq 
%		\displaystyle\sum\nolimits_{i = 1}^n 
%		\reward_i\curchoice.
%	\end{align*}
%	where $
%		\displaystyle\sum\nolimits_{i = 1}^n 
%		\reward_i\curchoice$
%		is the right hand side of the dual constraint corresponding to the
%		primal variable $\curalloc$.
%	Having this inequality,

\vspace{1mm}

\noindent\emph{\rom{2}. Comparing objective values of primal and dual.}
%By the fact that $\frac{A + B}{C + D} \geq \min\{\frac{A}{C} , \frac{B}{D}\}$,
We consider the contribution of each product $i$ in primal and dual 
(i.e. $\text{Primal}_{i}$ and $\text{Dual}_{i}$)
at each realization 
separately.
%The contributions of product in primal and dual for any fixed realization
%are as follows, 
Recall $\texttt{alloc}_i$ is the set of time periods when
a unit of product $i$ has been selected,
\begin{align*}
\text{Primal}_i &= 
\reward_i
%\left(
\displaystyle\sum\nolimits_{t = 1}^\totaltime
\indicator{\text{product $i$ is selected at time $t$}}
%\right)
\\
&= \reward_i|\texttt{alloc}_i| \\
\text{Dual}_i &= 
\reward_i
\displaystyle\sum\nolimits_{t = 1}^\totaltime 
\left(
\pen\left(\frac{\curinventorya}{\inventory_i}\right) 
+
\inventory_i\left(\pen\left(\frac{\curpseudoinventory}{\inventory_i}\right) 
-
\pen\left(\frac{\curpseudoinventory - 1}{\inventory_i}\right) \right)
\right)
\indicator{\text{product $i$ is selected at time $t$}} \\
&=
\reward_i
\displaystyle\sum\nolimits_{t \in \texttt{alloc}_i} 
\left(
\pen\left(\frac{\curinventorya}{\inventory_i}\right) 
+
\inventory_i\left(
\pen\left(\frac{\curpseudoinventory}{\inventory_i}\right) 
-
\pen\left(\frac{\curpseudoinventory - 1}{\inventory_i}\right) \right)
\right)
\end{align*}
Consider decreasing and concave function $\bar\pen(x) = \pen(1 - x)$,
by \emph{Global Dominance} of IAP assignment,
\begin{align*}
\sum_{t\in \texttt{alloc}_i}
	\pen\left(\frac{\curpseudoinventory}{\inventory_i}\right)  
	&=
\sum_{t\in \texttt{alloc}_i}
	\pen\left(\frac{\inventory_i - \assign_{i, t}}{\inventory_i}\right)   
	=
\sum_{t\in \texttt{alloc}_i}
\bar\pen\left(\frac{ \assign_{i,t}}{\inventory_i}\right)  
\geq 
\sum_{t\in \texttt{alloc}_i}
\bar\pen\left(\frac{\inventory_i - \curinventorya}{\inventory_i}\right)  
	=
\sum_{t\in \texttt{alloc}_i}
	\pen\left(\frac{\curinventorya}{\inventory_i}\right)   
\intertext{Hence,}
\text{Dual}_i &\leq 
\reward_i
\displaystyle\sum\nolimits_{t \in \texttt{alloc}_i} 
\left(
\pen\left(\frac{\curpseudoinventory}{\inventory_i}\right) 
+
\inventory_i\left(
\pen\left(\frac{\curpseudoinventory}{\inventory_i}\right) 
-
\pen\left(\frac{\curpseudoinventory - 1}{\inventory_i}\right) \right)
\right)
\end{align*}
Now, we partition time periods in $\texttt{alloc}_i$ into subgroups $A_{i, 1}, A_{i, 2}, \dots, A_{i, m}$ 
defined by \emph{Partition Monotonicity}
of IAP assignment, and consider the contribution of each subgroup $A_{i, k}$ in primal and dual 
(i.e. $\text{Primal}_{A_{i, k}}$ and $\text{Dual}_{A_{i, k}}$)
separately.
Recall that \emph{Partition Monotonicity} guarantees that 
$\{\assign_{i, t}:t \in A_{i, k}\} = \{1, 2, \dots, |A_{i, k}|\}$,
thus,
$\{\curpseudoinventory:t \in A_{i, k}\} 
= \{\inventory_i - |A_{i, k}| + 1, \inventory_i - |A_{i, k}| + 2, \dots, \inventory_i\}$.
Thus, let $x = \frac{\inventory_i - |A_{i, k}|}{\inventory_i}$,
\begin{align*}
\text{Primal}_{A_{i, k}} &= \reward_i \inventory_i (1-x) \\
\text{Dual}_{A_{i, k}} 
&\leq 
\reward_i \sum_{I = \inventory_i x + 1}^{\inventory_i}
\left(
\pen\left(\frac{I}{\inventory_i}\right) 
+
\inventory_i\left(
\pen\left(\frac{I}{\inventory_i}\right) 
-
\pen\left(\frac{I- 1}{\inventory_i}\right) \right)
\right) \\
&= 
\reward_i 
\sum_{I = \inventory_i x + 1}^{\inventory_i}
\pen\left(\frac{I}{\inventory_i}\right) 
+
\reward_i\inventory_i\left(
\pen(1) - 
\pen\left(x
%\frac{x}{\inventory_i}
\right)
\right)
\intertext{
Since $\pen(1) = 1$ and $\pen$ is increasing, it implies}
\sum_{I = \inventory_i x + 1}^{\inventory_i}
\pen\left(\frac{I}{\inventory_i}\right) 
&=
1 + 
\sum_{I = \inventory_i x + 1}^{\inventory_i - 1}
\pen\left(\frac{I}{\inventory_i}\right) \leq 
1 + 
\int_{x+\frac{1}{\inventory_i}}^1
\pen(y)\,dy
\intertext{
Thus,
}
\text{Dual}_{A_{i, k}} &\leq 
\reward_i\inventory_i\left(
\frac{1}{\inventory_i} + \int_{x+\frac{1}{\inventory_i}}^1
\pen(y)\,dy
+
1 -
\pen\left(
x
%\frac{x}{\inventory_i}
\right)
\right)
\intertext{and}
\frac{\text{Primal}_{A_{i, k}}}
{\text{Dual}_{A_{i, k}}} 
&\geq
\frac{1 - x}
{
\frac{1}{\inventory_i} + \int_{x+\frac{1}{\inventory_i}}^1
\pen(y)\,dy
+
1 -
\pen\left(
x
\right)
}
\end{align*}
Thus, we finish showing that 
\begin{align*}
\frac{\text{Primal}}
{\text{Dual}} 
&\geq
\min_{i \in [n]}
\frac{\text{Primal}_i}
{\text{Dual}_i}  
\geq
\min_{i \in [n]}
\min_{A_{i, k}}
\frac{\text{Primal}_{A_{i, k}}}
{\text{Dual}_{A_{i, k}}}   \\
&\geq
\GNRbound.
\end{align*}
Invoking \Cref{lem:random primal-dual} finishes the proof.
\end{proof}


==> tex/adversarial.tex <==
\label{sec:adversarial}
In this section, we consider the scenario with prior-free types 
when rental fees $\{\reward_i\}_{i\in[n]}$ and rental time 
$\{\duration_i\}_{i\in[n]}$ are deterministic and 
identical across time. 
The special case when consumers can only buy the products, i.e., they have infinite rental times, 
is studied in~\citet{GNR-14}. 
They propose a family of algorithms called \emph{Inventory-Balancing (IB)}, 
which are parameterized by a concave monotone non-decreasing \emph{penalty function} 
$\pen:[0, 1] \rightarrow [0, 1]$, satisfying $\pen(0) = 0$ and $\pen(1) = 1$. Roughly speaking, Inventory-Balancing is a myopic policy when the penalty function discounts the marginal revenue of each product as its inventory level drops. \citet{GNR-14} shows that Inventory-Balancing can achieve an asymptotic optimal competitive ratio of $\left(1-\frac{1}{e}\right)$ against an offline LP benchmark when initial inventories are large and the penalty functions is chosen appropriately, e.g., an exponential function.\footnote{Notably, both the algorithm and the analysis are adaptations of the Balance algorithm and its primal-dual analysis for AdWords problem~\citep{MSVV-05} to online assortment optimization.}

We extend the above results by showing that in the more general setting with fixed rental times over time, Inventory-Balancing achieves \emph{exactly} the same competitive ratio against our offline expected LP benchmark (\Cref{sec:alg} and \Cref{sec:exp-inventory-balancing}). The importance of this result is twofold. On one hand it shows the robustness of the Inventory-Balancing algorithm of \citet{GNR-14} when rentals are allowed. On the other hand, it emphasizes that by choosing an appropriate penalty function, the worst-case guarantee of myopic policy with discounted revenues improves from $50\%$ to $1-\tfrac{1}{e}\approx 63\%$ 
when inventories are large, which is also asymptotically optimal. 

We further extend our approach to i.i.d.\ stochastic rental times
and recover the same competitive ratio but against a LP defined on the reverse order of type sequence, which implies $(1-\tfrac{1}{e})^2$-competitive
against proposed revenue optimal offline LP benchmark. More details are provided in \Cref{sec:stochastic-prior-free}.
%The latter improves the result of \cite{GGISUW-19}.


%their results that in this more general setting
%with identical rental duration distribution,
%a losser but 
%tight in extreme 
%(initial inventory is one for some products
%or 
%sufficient large for all products) 
%%the same
%constant competitive ratio guarantee holds.
\subsection{Inventory-Balancing and Competitive Ratios for Fixed Rental Times}
\label{sec:alg}
Recall the sequence of events at each time period $t$:
\begin{enumerate}
 \linespread{1}
\item For each product $i$, a number of rental units of this product return to inventory. We denote the inventory level of product $i$ at this moment as $\curinventorya$.
\vspace{-3mm}
\item Consumer $t$ arrives and the platform realizes her $\type_t$.
\vspace{-3mm}
\item Platforms offers an assortment $\assortment_t$ to consumer $t$.
\vspace{-3mm}
\item The exact choice of the consumer $i_t$ and her rental time $d_{i_t}\sim\durationdistribution_{i_t}$ are realized.
\end{enumerate}
In this section, we focus on the case where rental time of each product is fixed over time, hence $\{d_i\}_{i=1}^n$ are known upfront. \Cref{alg:IB} describes the Inventory-Balancing policy with penalty function $\pen(.)$ when rentals are allowed. 




%(we denote the inventory level of product $i$ at this point as 
%$\curinventoryb$).




\begin{algorithm}
	\caption{Inventory-Balancing with penalty function $\pen$  \citep{GNR-14}}
	\label{alg:IB}
	\begin{algorithmic}[1]
	\vspace{+2mm}
		\For{each consumer $t \in [T]$ with type $\type_t$}
		\State Update all inventory levels $\{\curinventorya\}$, considering rental products that return at time $t$.
		\State Offer assortment 
		$\assortment_t 
		= \argmax_{\assortment \in \assortmentspace} 
		\displaystyle\sum\nolimits_{i = 1}^n \reward_i\curchoice\curpenA$.
		\EndFor
	\end{algorithmic}
\end{algorithm}

By substitutability (\Cref{asp:substitutability}), 
and the fact that $\pen(0) = 0$, 
assortments offered by IB are inventory feasible. Now, we have the main theorem of this section that bounds the competitive ratio of IB against the expected LP benchmark when rental times are fixed over time.

\begin{theorem}
	\label{thm:concave competitive ratio}
	In prior-free online assortment optimization where each product 
	has deterministic and identical rental fee and
rental time, 
	for any monotone non-decreasing, concave and differentiable
	penalty function $\pen$,
	the competitive ratio of the 
	Inventory-Balancing algorithm against $\EAR{\typesequence}$ is at least 
	$\GNRnotation$, where
	\begin{align*}
		\GNRnotation = \GNRbound~,
	\end{align*}
$\mininventory = \min_{i\in[n]}\inventory_i$ is the smallest initial inventory.
\end{theorem}
\begin{corollary}[similar to \cite{GNR-14}]
\label{cor:gnr-bounds}
 For any monotone non-decreasing and concave penalty function $\pen$ in $(0,1]$, the competitive ratio in \Cref{thm:concave competitive ratio} is at least $\%50$. 
 Moreover, the optimal competitive ratio is obtained by  exponential penalty function $\exponential$, which approaches to $\left(1-\sfrac{1}{e}\right)\approx \%63$ as $\mininventory$ increases to infinity.

\end{corollary}

\begin{remark}
IB does not keep track of the full state of 
rentals, i.e., how many units of each product are on-hand and when rented units return. Also, it does not exploit the knowledge of rental times of different products; nevertheless, it always obtains a constant competitive ratio of at least $\%50$.
\end{remark}

The proof of \Cref{thm:concave competitive ratio} is done using a new \emph{primal-dual analysis} (which at high-level resembles the primal-dual analysis of \citet{MSVV-05} for online budgeted allocation or its adaption in \cite{GNR-14} for online assortment optimization with no rentals). Our analysis diverges from past work as inventory level of an arbitrary product is not decreasing anymore due to rentals, which is a critical property needed in previous analysis. 

To address this challenge, we come up with a modified randomized dual construction. For the general concave penalty functions, the construction is rather involved; it uses a chain of techniques to reduce the problem of finding an appropriate dual assignment to solving a sub-problem called  \emph{interval assignment problem}.  We defer the details of this reduction and how to solve this sub-problem to \Cref{app:general-penalty}. Instead, here we prove a weaker version of \Cref{thm:concave competitive ratio} for the special case of \emph{Exponential Inventory-Balancing (EIB)} algorithm, which is IB with penalty function $\exponential$.



 
%(which is rather involved for general inventory balancing, see \Cref{app:general-penalty}). 
%Second, we establish our dual construction based on the modified reverse-order expected LP; as will be see in the Proof of \Cref{thm:exponential competitive ratio} and Proof of \Cref{thm:concave competitive ratio}, this modification is critical to finish our primal-dual analysis. Finally, 
\begin{proposition}
	\label{thm:exponential competitive ratio}
	Let $\mininventory = \min_{i\in[n]}\inventory_i$
	be the smallest initial inventory.
	In prior-free online assortment optimization with fixed over time rental times, the competitive ratio of the 
	Exponential Inventory-Balancing (EIB) algorithm is at least 
	$\exponentialbound$ against $\EAR{\typesequence}$,
	which approaches to $(1-\sfrac{1}{e})$ as $\mininventory$ increases to infinity.
\end{proposition}


The competitive ratio of EIB in \Cref{thm:exponential competitive ratio} does not depend
on the rental time or the fee for each product. It is asymptotic tight in sense that no online algorithm can obtain a competitive ratio better than $(1 - \sfrac{1}{e})$ if the duration is always infinite \citep[cf.][]{GNR-14}.


\subsection{Analysis of Exponential Inventory-Balancing: Proof of \Cref{thm:exponential competitive ratio}}
\label{sec:exp-inventory-balancing}

For a fixed sequence of consumer types $\typesequence$, consider 
$\EAR{\typesequence}$ defined in \Cref{sec:prelim}. Our dual construction is randomized and produces a dual assignment that is only feasible in expectation. Interestingly, this is enough for our analysis because of the following technical lemma.

\begin{lemma}[\citealp{DJK-13}]
	\label{lem:random primal-dual}
	Suppose a randomized primal-dual algorithm constructs a feasible primal assignment with value $P$ 
	(which is a random variable) and
	a dual assignment (not necessarily feasible) with value
	$D$ (which is also a random variable), such that
	\begin{enumerate}
		\item For some  constant $\alpha$, it always holds that $P \geq \alpha\cdot D$~,
			
		\item The expectations of the randomized dual assignments form a feasible dual solution.
	\end{enumerate}
Then, the expectation of $P$ is at least $\alpha \cdot {\OPT}$ where $\OPT$ is the value of the optimum solution.
\end{lemma}


We are now ready to present our primal-dual analysis for the simpler case of EIB. 
\begin{proof}[Proof of \Cref{thm:exponential competitive ratio}]
	Consider the following primal linear program, i.e., $\EAR{\typesequence}$:
	\begin{align*}
		%\nonumber
		&\begin{array}{rlll}
		\max
		\limits_{\mathbf \alloc \geq \mathbf 0} &
		\displaystyle\sum\nolimits%\limits
		_{t=1}^\totaltime
		\displaystyle\sum\nolimits%\limits
		_{\assortment \in \assortmentspace}
		\displaystyle\sum\nolimits%\limits
		_{i=1}^n
		\reward_i\curchoice\curalloc
		&
		\text{s.t.}
		&\\ %& & &\\
		&
		\displaystyle\sum\nolimits_{\tpre = 1}^{t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
		%(1-\durationdistribution_i(t - \tpre)) 
		%\prob[\durationdistribution_i]{\duration_{i, \tpre} \geq \tpre - t}
		\durationcdfi_i(t-\tpre)
		\prechoice\prealloc \leq \inventory_i
		& i \in [n],\ t \in [\totaltime]
		%\forall i\in[n],t \in [T] 
		&\langle\inventorydual\rangle
		\\
		&\displaystyle\sum\nolimits_{\assortment\in \assortmentspace}\curalloc \leq 1
		&t \in [\totaltime]
		&\langle\probdual\rangle \\
	%\end{array}\\
		\intertext{Since the rental times are deterministic, we can rewrite the primal program as}
		\max
		\limits_{\mathbf \alloc \geq \mathbf 0} &
		\displaystyle\sum\nolimits%\limits
		_{t=1}^\totaltime
		\displaystyle\sum\nolimits%\limits
		_{\assortment \in \assortmentspace}
		\displaystyle\sum\nolimits%\limits
		_{i=1}^n
		\reward_i\curchoice\curalloc
		&
		\text{s.t.}
		&\\ %& & &\\
		&
		\displaystyle\sum\nolimits_{\tpre = t}^{\min\{t + \duration_i - 1,\totaltime\}}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
		%(1-\durationdistribution_i(t - \tpre)) 
		%\prob[\durationdistribution_i]{\duration_{i, \tpre} \geq \tpre - t}
		\prechoice\prealloc \leq \inventory_i
		& i \in [n],\ t \in [\totaltime]
		%\forall i\in[n],t \in [T] 
		&\langle\inventorydual\rangle
		\\
		&\displaystyle\sum\nolimits_{\assortment\in \assortmentspace}\curalloc \leq 1
		&t \in [\totaltime]
		&\langle\probdual\rangle \\
	\intertext{We then construct its dual program with dual variables $\inventorydual$ 
	and $\probdual$ as follows:} 
		%\nonumber
	%	&\begin{array}{rlll}
		\min
		\limits_{\boldsymbol{\theta},\boldsymbol{\lambda} \geq \mathbf 0} &
		\displaystyle\sum\nolimits%\limits
		_{t=1}^\totaltime
		\displaystyle\sum\nolimits%\limits
		_{i=1}^n
		\inventory_i\inventorydual
		+
		\displaystyle\sum\nolimits_{t =1}^\totaltime
		\probdual
		& 
		\text{s.t.} 
		&\\ %& & &\\
		&
		\probdual + 
		\displaystyle\sum\nolimits_{i = 1}^n
		\displaystyle\sum\nolimits_{\tpre= \max\{t - \duration_i + 1, 1\}}^t
		%(1-\durationdistribution_i(t - \tpre)) 
		%\prob[\durationdistribution_i]{\duration_{i, \tpre} \geq t - \tpre}
		\curchoice\theta_{i,\tpre}
	 %& & \\
%				&  
%		\qquad\qquad
%		\qquad\qquad
%		\qquad\qquad
%		\qquad\qquad
		\geq \displaystyle\sum\nolimits_{i = 1}^n
		\reward_i\curchoice
		& \assortment \in \assortmentspace,\ t \in [\totaltime]
		%\forall i\in[n],t \in [T] 
		&\langle\curalloc\rangle
	\end{array}
\end{align*}	
	Let $\assortment_t$ be the assortment offered to consumer $t$.
	Recall $\curinventorya$ 
	%(resp.\ $\curinventoryb$) 
	is the 
	inventory level of product $i$ at time period $t$ 
	before 
	%(resp.\ after) 
	the realization of 
	consumer selection. 
	%For notation simplicity, we denote $\curpenA$ and $\curpenB$ as 
	%$\curpena$ and $\curpenb$, respectively.
	Consider the following assignments of primal (which is deterministic) and dual (which is randomized):
	\begin{align*}
		\textit{Primal:}~~~~~\curalloc &= \indicator{\assortment_t = \assortment},\\
		\textit{Dual:}~~~~~~~ \probdual &= \displaystyle\sum\nolimits_{i = 1}^n \reward_i 
		\pen\left(\frac{\curinventorya}{\inventory_i}\right)
		\cdot
			\indicator{\text{product $i$ is selected at time $t$}},\\
			~~~~~~~~\inventorydual &= \reward_i\left(
			\pen\left(\frac{\curinventorya}{\inventory_i}\right) -
			\pen\left(\frac{\curinventorya - 1}{\inventory_i}\right)
			\right) 
			\cdot
			\indicator{\text{product $i$ is selected at time $t$}}
	\end{align*}
	where 
		$\indicator{\cdot}$ is an indicator operator. Note that product $i$ is selected at time $t$ if it belongs to the assortment set $\assortment_t$ and consumer arriving at time $t$ chooses this product.  In the rest of analysis, we show the above randomized primal-dual assignments satisfy the conditions of \Cref{lem:random primal-dual} for 
		$\alpha =\exponentialbound$,
		which finishes the proof.
	\vspace{1mm}

	\noindent\emph{\rom{1}. Primal feasibility and dual feasibility in expectation.}
 The primal assignment is feasible, as EIB (and in general any member of the IB family) only offers inventory feasible assortments. To show dual feasibility in expectation, first note that $\pen(.)$ is non-negative and monotone non-decreasing. 
 Therefore $\probdual\geq 0$ for all $t\in[\totaltime]$, and $\inventorydual\geq 0$ for all $i\in[n],t\in[\totaltime]$. 
 Next, we show for every $t\in[\totaltime]$ and $\assortment\in\assortmentspace$, 
 the dual assignment satisfies the dual constraints corresponding to $\curalloc$ in expectation. 
 %Let $\indicator{\duration_{i, \tpre} \geq t - \tpre}$ be the indicator of the event that rental time of product $i$ at time $\tpre$ is at least 
	%$t - \tpre$. 
	For every product $i\in[n]$, the following inequality holds at every time $t\in[\totaltime]$: 
	\begin{align}
		\label{eq:dual feasible ex post}
		\reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right) 
		+ \displaystyle\sum\nolimits_{\tpre = \max\{t-\duration_i + 1, 1\}}^{t - 1}
		\theta_{i, \tpre} 
		\geq \reward_i
	\end{align}
	To see why inequality~\eqref{eq:dual feasible ex post} holds, consider on-hand units and under rental units of product $i$ at time $t$. Since the inventory level of product $i$ at time $t$ is 
	$\curinventorya$, there are $\inventory_i - \curinventorya$ units of product $i$ under rental at that moment. Suppose these units were rented at times
	$\tpre_1\leq\tpre_2\leq \dots\leq\tpre_{\inventory_i - \curinventorya}$,
	where $\max\{t-\duration_i + 1, 1\} \leq \tpre_j \leq t - 1$ and 
	$\indicator{\text{product $i$ is selected at time $\tpre_j$}} = 1$
	for all $j\in[\inventory_i - \curinventorya]$.
	Additionally, the inventory level at time $\tpre_j$ is at most $\inventory_i - j + 1$,
	i.e.,
	$I_{i, \tpre_j} \leq \inventory_i - j + 1$ for all $j \in [\inventory_i - \curinventorya]$. This is true because at time $\tau_j$ at least $j-1$ units of the product are under rental due to rents happening at $\tau_1,\ldots,\tau_{j-1}$.
Because the penalty function $\pen(\cdot)$ is concave, we have:
	\begin{align}
	\label{eq:concave}
		\theta_{i, \tpre_j} = 
		\reward_i\left(\pen\left(\frac{I_{i, \tpre_j}}{\inventory_i}\right)
		-
	\pen\left(\frac{I_{i, \tpre_j} - 1}{\inventory_i}\right)\right)
		\geq
		\reward_i\left(\pen\left(\frac{\inventory_i - j + 1}{\inventory_i}\right)
		-
	\pen\left(\frac{\inventory_i - j}{\inventory_i}\right)\right)
	\end{align}
By applying \eqref{eq:concave},  we can prove inequality~\eqref{eq:dual feasible ex post}:
\begin{align*}
&\quad~\reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right) 
		+ \displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,1\}}^{t - 1}	\theta_{i, \tpre}\\
		& \geq\reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right) 
		+ \displaystyle\sum\nolimits_{j = 1}^{\inventory_i - \curinventorya} \reward_i\left(\pen\left(\frac{I_{i, \tpre_j}}{\inventory_i}\right)
		-
	\pen\left(\frac{I_{i, \tpre_j} - 1}{\inventory_i}\right)\right)\\
	&\geq \reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right) + \displaystyle\sum\nolimits_{j = 1}^{\inventory_i - \curinventorya} \reward_i\left(\pen\left(\frac{\inventory_i - j + 1}{\inventory_i}\right)
		-
	\pen\left(\frac{\inventory_i - j}{\inventory_i}\right)\right)\\
	&=\reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right) +\displaystyle\sum\nolimits_{I = \curinventoryb}^{\inventory_i - 1} 
		\reward_i\left(
			\pen\left(\frac{I + 1}{\inventory_i}\right) 
			-
			\pen\left(\frac{I}{\inventory_i}\right) 
		\right)=\reward_i\pen(1)=\reward_i
\end{align*}	
%	we start with the following equality,
%	\begin{align*}
%		1 = \pen(1) = \displaystyle\sum\nolimits_{I = \curinventoryb}^{\inventory_i - 1} 
%		\left(
%			\pen\left(\frac{I + 1}{\inventory_i}\right) 
%			-
%			\pen\left(\frac{I}{\inventory_i}\right) 
%		\right) 
%		+
%		\pen\left(\frac{\curinventoryb}{\inventory_i}\right) 
%	\end{align*}
%	
%	we start with the following equality,
%	\begin{align*}
%		1 = \pen(1) = \displaystyle\sum\nolimits_{I = \curinventoryb}^{\inventory_i - 1} 
%		\left(
%			\pen\left(\frac{I + 1}{\inventory_i}\right) 
%			-
%			\pen\left(\frac{I}{\inventory_i}\right) 
%		\right) 
%		+
%		\pen\left(\frac{\curinventoryb}{\inventory_i}\right) 
%	\end{align*}
%	
%	

Now, for each time $t\in[\totaltime]$ and assortment $\assortment\in\assortmentspace$, consider the following expression:
	\begin{align}
		\label{eq:dual LHS}
		\probdual + 
		\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,1\}}^t
		\curchoice \theta_{i, \tpre} 
	\end{align}
On the one hand, note that by taking expectation from \eqref{eq:dual LHS} we have 
\begin{equation}
\label{eq:first-compare}
\expect{\probdual + 
		\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,1\}}^t
		\curchoice \theta_{i, \tpre} }=\expect{\probdual} + 
		\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,1\}}^t
		\curchoice \expect{\theta_{i, \tpre}} ~,
\end{equation}
simply because of linearity of expectation. On the other hand, by taking expectation from \eqref{eq:dual LHS} by first conditioning on (i) history up to time $t$ (which includes inventory levels $\curinventorya$ for each product $i$), and (ii) assortment $\assortment_t$ offered at time $t$, we have
	%(notice that this is independent of all events before $t$ or 
	%the assortment $\assortment_t$ offered at time $t$ or 
	%the inventory level at time $t$),
	\begin{align}
		&\expect{\probdual + 
		\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,1\}}^t
		\curchoice \theta_{i, \tpre} |\mathcal{F}_{t-1},\assortment_t}\nonumber\\
		&~~=\displaystyle\sum\nolimits_{i = 1}^n 
		\reward_i\choice^{\type_t}(\assortment_t, i)
		\pen\left(\frac{\curinventorya}{\inventory_i}\right)
		+	
		\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,1\}}^{t - 1}
		\curchoice \theta_{i, \tpre} \nonumber \\
		 &~~+
		\displaystyle\sum\nolimits_{i = 1}^n 
		\choice^{\type_t}(\assortment, i)\reward_i
		\choice^{\type_t}(\assortment_t, i)
		\left(
		\pen\left(\frac{\curinventorya}{\inventory_i}\right)
		-
		\pen\left(\frac{\curinventorya - 1}{\inventory_i}\right)
		\right)\label{eq:third-term}\\
		&~~\overset{(a)}{\geq} 
	\displaystyle\sum\nolimits_{i = 1}^n 
		\reward_i\curchoice
		\pen\left(\frac{\curinventorya}{\inventory_i}\right)
		+	
		\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,1\}}^{t - 1}
		\curchoice \theta_{i, \tpre}\nonumber  \\
		&~~=\displaystyle\sum\nolimits_{i = 1}^n 
		\curchoice\left(\reward_i\pen\left(\frac{\curinventorya}{\inventory_i}\right)+ \displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,1\}}^{t - 1}
		\theta_{i, \tpre}  \right)
		\nonumber \\
		&~~\overset{(b)}{\geq} \displaystyle\sum\nolimits_{i = 1}^n 
		\reward_i\curchoice~,\nonumber
	\end{align}
where $\mathcal{F}_{t-1}$ denotes the history up to time $t$. Note that inequality~(a) above holds because $$
		\assortment_t = 
		\argmax_{\assortment \in \assortmentspace}\displaystyle\sum\nolimits_{i = 1}^n\reward_i\curchoice
		\pen\left(\frac{\curinventorya}{\inventory_i}\right)~,
		$$
and the third term in expression~\eqref{eq:third-term} is non-negative, and inequality~(b) holds because of  inequality~\eqref{eq:dual feasible ex post}. Therefore, by taking another expectation over $\assortment_t$ and  $\mathcal{F}_{t-1}$, we have:
\begin{equation}
\label{eq:second-compare}
\expect{\probdual + 
		\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = \max\{t-d_i+1,1\}}^t
		\curchoice \theta_{i, \tpre} }\geq \displaystyle\sum\nolimits_{i = 1}^n 
		\reward_i\curchoice
\end{equation}
Combining \eqref{eq:first-compare} and \eqref{eq:second-compare} shows  feasibility in expectation of the dual assignment.
%	\begin{align}
%		\label{eq:dual feasible ex post final}
%		\eqref{eq:feasibility ex post} 
%		\geq 
%		\displaystyle\sum\nolimits_{i = 1}^n 
%		\reward_i\curchoice
%		\pen\left(\frac{\curinventorya}{\inventory_i}\right)
%		&+	
%		\displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre = 1}^{t - 1}
%		\indicator{\duration_{i, \tpre} \geq t - \tpre}
%		\curchoice \theta_{i, \tpre}  
%	\end{align}
%	Applying inequality \eqref{eq:dual feasible ex post}, it implies
%	\begin{align*}
%		\eqref{eq:feasibility ex post} 
%		\geq 
%		\displaystyle\sum\nolimits_{i = 1}^n 
%		\reward_i\curchoice.
%	\end{align*}
%	where $
%		\displaystyle\sum\nolimits_{i = 1}^n 
%		\reward_i\curchoice$
%		is the right hand side of the dual constraint corresponding to the
%		primal variable $\curalloc$.
%	Having this inequality,
	
	\vspace{1mm}
	
	\noindent\emph{\rom{2}. Comparing objective values of primal and dual.} We consider the value increments in both primal and dual for each time period separately. Conditioned on history up to time $t$ and offering assortment $\assortment_t$ at time $t$, the expected increments (over randomness of the choice of consumer $t$) in primal and dual are
	\begin{align*}
		\expect{\Delta(\text{Primal})|\mathcal{F}_{t-1},\assortment_t}&= \displaystyle\sum\nolimits_{i = 1}^n r_i\choice^{\type_t}(\assortment_t, i) \\
		\expect{\Delta(\text{Dual})|\mathcal{F}_{t-1},\assortment_t} &= \displaystyle\sum\nolimits_{i = 1}^n r_i\choice^{\type_t}(\assortment_t, i)
		\pen\left(\frac{\curinventorya}{\inventory_i}\right)
		+ \displaystyle\sum\nolimits_{i = 1}^n \inventory_i
		\reward_i
		\choice^{\type_t}(\assortment_t, i)
		\left(
			\pen\left(\frac{\curinventorya}{\inventory_i}\right)
			-
			\pen\left(\frac{\curinventorya - 1}{\inventory_i}\right)
		\right)
	\end{align*}
	Thus, to show $\expect{\textrm{Obj(Primal)}}\geq \alpha \cdot\expect{\textrm{Obj(Dual)}}$ it is sufficient to show
	\begin{align}
		\label{eq:increament}
	\pen\left(\frac{\curinventorya}{\inventory_i}\right)
			+
		\inventory_i 
		\left(
			\pen\left(\frac{\curinventorya}{\inventory_i}\right)
			-
			\pen\left(\frac{\curinventorya- 1}{\inventory_i}\right)
		\right)\leq \tfrac{1}{\alpha}
	\end{align}
%	We provide two different arguments to upperbound \eqref{eq:increament}, which results in
%	$\alpha=\frac{1}{2}$ and $\alpha=\exponentialbound$, respectively.
%\vspace{1mm}
%
%	\emph{Case 1 ($\alpha=\sfrac{1}{2}$):} 
%	We start with an observation purposed by \citet{GGISUW-19}: it is without 
%	loss of generality to assume $\inventory_i = 1$ for each product $i$. Guarantees for the case of unit inventory leads to a stronger result that generalizes to the case of arbitrary inventories. To see this, consider a unit inventory setting where for each product $i$ we have $\inventory_i$ identical products, each with an inventory of $1$,
%	instead of $\inventory_i$ units of product $i$ in the original instance. The revenue of our benchmark remains unchanged and any algorithm for the unit inventory case can be used for arbitrary inventory case without loss in revenue. Due to the fact that the penalty function $\pen$ is increasing with $\pen(0) = 0$ and $\pen(1) = 1$, when $\inventory_i = 1$,
%	\begin{align*}
%		\textrm{LHS of}~\eqref{eq:increament} \leq \pen(1) + \inventory_i (\pen(1) - \pen(0)) \leq 2
%	\end{align*}
%	\vspace{1mm}
The exponential penalty function $\exponential$ satisfies the following differential equation:
	$$\pen'(x) +\pen(x)= \frac{e}{e-1}$$.
Therefore, we have:
	\begin{align*}
		\textrm{LHS of}~\eqref{eq:increament}  &\overset{(a)}{\leq} 
		\pen\left(
			\frac{\curinventorya}{\inventory_i}
		\right) 
		+
		\left(
			\curinventorya - (\curinventorya - 1)
			\right)
		\pen'\left(
			\frac{\curinventorya - 1}{\inventory_i}
		\right)  \\
		&\overset{(b)}{=} 
		\frac{e}{e - 1} + 
		\pen\left(
			\frac{\curinventorya}{\inventory_i}
		\right)  -
		\pen\left(
			\frac{\curinventorya-1}{\inventory_i}
		\right) 
		\\
		&\overset{(c)}{\leq}  \frac{e}{e - 1} +\pen(\frac{1}{\inventory_i})-\pen(\frac{0}{\inventory_i})\\
		&= 
		\frac{e}{e - 1} +
		\frac{e - e^{1 - \sfrac{1}{\inventory_i}}}{e - 1} 
		\leq 
		\frac{2e - e^{1 - \sfrac{1}{\mininventory}}}{e - 1}=\frac{1}{\alpha}
	\end{align*}
where both~(a) and (c) hold due to concavity of $\pen$, and~(b) holds as $\pen'(x)=\tfrac{e}{e-1}-\pen(x)$.
\end{proof}

%Note that in the proof of \Cref{thm:exponential competitive ratio}, concavity and monotonicity of $\pen(.)$ are the only properties used to prove $\alpha=\tfrac{1}{2}$. Thus, with the same argument,
%$\sfrac{1}{2}$-competitive guarantee against expected LP benchmark is preserved  for general concave and monotone penalty functions, which improves the $\tfrac{1}{2}$-competitive shown in \cite{GGISUW-19} against the weaker clairvoyant benchmark.

%\begin{corollary}
%	\label{prop:concave penalty}
%%	The competitive ratio of Inventory-Balancing algorithm
%	with arbitrary non-decreasing concave penalty function $\pen$
%	is at least $\sfrac{1}{2}$ against $\EAR{\inversetypesequence}$. Specifically, 
%	the greedy myopic algorithm defined by $\pen(x)=\indicator{x>0}$ 
%	is $\sfrac{1}{2}$-competitive.
%\end{corollary}

\subsection{Stochastic i.i.d. Rental Times}
\label{sec:stochastic-prior-free}
So far we have shown that when rental times are stationary and deterministic IB policies obtain \emph{exactly} the same competitive ratio against the offline expected LP as in the case with no rentals. Can we obtain a similar result for the stochastic i.i.d. rental times with general duration distributions? We answer this question in affirmative by showing IB remains to be constant competitive against the offline expected LP benchmark even in the stochastic setting. Our approach obtains a weaker guarantee compared to the fixed duration setting, which leaves tightening the gap for competitive guarantee of IB in this setting as an interesting open question.


The new key technical ingredient in our analysis for the stochastic setting is using a \emph{modified} version of our expected LP benchmark $\EAR{\typesequence}$ named as \emph{reverse expected LP}. This linear program is exactly as our previous expected LP benchmark, but considers consumer types in the reverse order, i.e., $\EAR{\inversetypesequence}$ where $\type'_t = \type_{T - t + 1}$. With this modification, the new program does not remain to be a revenue optimal benchmark anymore (as we can show through simple examples); however, it turns out that we can extend our previous primal-dual analysis and show that the expected revenue obtained by IB is at least a constant fraction of the optimal objective value of this LP. This is again done by constructing a randomized feasible assignment for the dual of this new program, so that expected revenue obtained by IB is at least a constant fraction of the objective value of this dual assignment. Formally, we have the following proposition. We defer its proof to \Cref{app:general-penalty}.

\begin{proposition}
	\label{prop:concave competitive ratio-iid}
	In prior-free online assortment optimization where each product has identical rental fee and stochastic i.i.d. rental times over time, 
	for any monotone non-decreasing, concave and differentiable
	penalty function $\pen$,
	the competitive ratio of the 
	Inventory-Balancing algorithm against $\EAR{\inversetypesequence}$ is at least 
	$\GNRnotation$, where
	\begin{align*}
		\GNRnotation = \GNRbound~,
	\end{align*}
$\mininventory = \min_{i\in[n]}\inventory_i$ is the smallest initial inventory and $\type'_t = \type_{T - t + 1}$.
\end{proposition}

\begin{remark} 
\label{remark:iid-fixed}
For the special case of deterministic rental times, the optimal objective value of the reverse expected LP  $\EAR{\inversetypesequence}$ \emph{exactly} matches  the objective value of expected LP benchmark $\EAR{\typesequence}$, simply because two programs have exactly the same set of constraints. Therefore, \Cref{prop:concave competitive ratio-iid} generalizes \Cref{thm:concave competitive ratio}.
\end{remark}

The main result of this section is an immediate corollary of \Cref{prop:concave competitive ratio-iid}.

\begin{theorem}
	\label{thm:concave competitive ratio-iid}
	In prior-free online assortment optimization where each product has identical rental fee and stochastic i.i.d. rental times over time, 
	for any monotone non-decreasing, concave and differentiable
	penalty function $\pen$,
	the competitive ratio of the 
	Inventory-Balancing algorithm against offline expected LP benchmark $\EAR{\typesequence}$ is at least 
	$$\beta_{\mininventory}(\Psi)\triangleq\underset{\Psi':[0,1]\rightarrow [0,1], \textrm{non-decreasing, concave}}{\max}\{\GNRnotation\cdot\alpha_{\mininventory}(\Psi')\}$$
In particular, $\beta_{\mininventory}(\Psi)\in [\tfrac{1}{4},(1-\tfrac{1}{e})^2]$, and $\underset{{\mininventory\rightarrow \infty}}{\lim}\beta_{\mininventory}(\Psi)=(1-\tfrac{1}{e})^2\approx \%40$ for $\exponential$.
\end{theorem}
\begin{proof} Because of \Cref{prop:concave competitive ratio-iid}, IB's expected revenue is at least $\GNRnotation$ fraction of the optimal objective value of the reverse expected LP. Moreover, if we run an IB policy with penalty function $\Psi'(.)$ on the reverse sequence of types, its expected revenue will be at least $\alpha_{\mininventory}(\Psi')$ fraction of the forward expected LP's optimal objective value. As the revenue of IB on the reverse sequence of types is upper-bounded by the reverse expected LP's optimal objective value (due to \Cref{lem:relaxation}), the expected revenue of IB on the forward sequence of types will be at least $\GNRnotation\cdot \alpha_{\mininventory}(\Psi')$ fraction of the optimal objective value of (forward) expected LP. This result holds for any concave and non-decreasing function $\Psi'(.):[0,1]\rightarrow [0,1]$, which finishes the proof.
\end{proof}


==> tex/apx-hardness.tex <==

\section{Unbounded Competitiveness of Optimum Offline}
\label{apx:hardness-optoffline}

In this section, we construct a simple instance
which
shows 
the Bayesian expected LP $\EAR{\typedistributionsequence}$
is at most a $O(\sfrac{1}{T})$-approximation to the optimum offline.
Combining with \Cref{prop:relaxation},
it implies that no online algorithm can achieve a ($T$-independent) bounded 
competitive ratio against optimum offline.

\begin{theorem}
\label{thm:hardness-optoffline}
The Bayesian expected LP $\EAR{\typedistributionsequence}$
is at most a $O(\sfrac{1}{T})$-approximation to the optimum offline.
\end{theorem}

\begin{corollary}
No online algorithm
can achieve a 
($T$-independent) 
bounded 
competitive ratio against optimum offline.
\end{corollary}

\begin{proof}{\emph{Proof of \Cref{thm:hardness-optoffline}.}}
Consider the following instance
where
there is a single product
and a single consumer type.
For this product, its initial inventory is one, 
reward is one.
Once this product is allocated, the realized rental duration 
is one (i.e., becoming available in the next time period) with probability $\sfrac{1}{2}$,
and infinite otherwise.
At every time period $t \in [T]$,
a consumer with this single consumer type arrives the platform
with probability one. 
Consumers select this product (if assorted) with probability one.

First, we claim that the expected revenue of the optimum offline
is at least $\sfrac{T}{2}$.
Note that the optimum offline observe the realization of rental
duration of
the product at each time period before assorting, and thus it can assort
the product whenever the realized rental duration at that time 
period is one. 
Since 
the expected number of such time period is $\sfrac{T}{2}$,
the expected revenue of optimum offline is at least $\sfrac{T}{2}$.

Next, we consider the Bayesian expected LP 
$\EAR{\typedistributionsequence}$
and its dual program on this instance:
\begin{equation*}
% \tag{\textsc{Primal-Dual-Upperbound}}
% \label{eq:LP-lower-bound}
\arraycolsep=1.4pt\def\arraystretch{1}
\begin{array}{llllllll}
\max\quad\quad\quad&
\displaystyle\sum_{t=1}^T
y_t
\qquad\qquad\qquad&\text{s.t.}&
&\quad\quad\text{min}\quad\quad\quad &
\displaystyle\sum_{t=1}^T
\theta_t
\qquad\qquad\qquad&\text{s.t.} \\[1.4em]
 &
 \displaystyle\sum_{\tau=1}^t{\frac{1}{2}\,y_\tau}\leq 1 & 
 t\in[T]~.
 & 
& &
 \displaystyle\sum_{\tau=t}^T{\frac{1}{2}\,\theta_\tau}\geq 1 & 
 t\in[T]~.
\end{array}
\end{equation*}
Consider the following feasible dual solution 
with objective value 2
in the dual program:
$$\theta_t = 0,~\forall t\in[T - 1], ~~~~ \theta_T = 2.$$
Invoking the weak duality between the above primal-dual linear
programs finishes 
the proof.
 \hfill\Halmos
\end{proof}

==> tex/apx-subassortment.tex <==
\subsection{Omitted Proof for Proposition~\ref{prop:assortment polytope}}
\label{apx:subassortment sampling}

\polytope*
\begin{proof}
% [Proof of \Cref{prop:assortment polytope}]
To show the polynomial 
running time,
observe that 
(a) the running time in each recursion
is $\textrm{Poly}(n)$;
and 
(b) the number of recursion is 
at most $|\assortment| \leq n$, 
since $\assortment'$ called in the recursion
satisfying that $|\assortment'| \leq |\assortment| - 1$.

Property (i) holds by construction.
We show property (ii) by induction on 
$m = |\assortment|$,
i.e., size of 
assortment $\assortment$. 
% Without loss of generality, we assume 
% $\sigma(i) = i$ for all $i \in \assortment$.
In this induction, 
we use another simple property (iii)
that
$\phi(\assortment, i)\left(\sum_{j=\sigma(i)}^m q_j\right)  = p_{i}$
for all $i\in \assortment$,
which immediately hold by construction.

\noindent\emph{Base Case ($m=1$).} 
In this case
Procedure~\ref{alg:sample assortment} randomly outputs
$\emptyset$ or $\assortment$.
By property (iii), the induction statement
holds.

\noindent\emph{Inductive step ($m > 1$).} 
Fix an arbitrary product $i\in \assortment$.
Notice that by construction
$
\expect[\tilde\assortment]{\choice(\tilde\assortment, i)
    \condition j^* < \sigma(i)} = 0$,
and 
$
\expect[\tilde\assortment]{\choice(\tilde\assortment, i)
    \condition j^* = m}
    =
    \choice(\assortment, i)$.
For any $j = i, \dots, m - 1$,
and $\assortment' = \{\sigma(k)\}_{k=1}^{j}$. 
Since the choice model $\choice$ is weak substitutable,
i.e., $\choice(S', i) \geq \choice(S, i)$,
invoking induction hypothesis on assortment $\assortment'$
with $|\assortment'| \leq m-1$, we have 
    $\expect[\tilde\assortment]{\choice(\tilde\assortment, i)
    \condition j^* = j} = \choice(\assortment, i)$ for all $j = i, \dots, m - 1$.
    Thus, invoking property (iii),
\begin{align*}
\expect[\tilde\assortment]{\choice(\tilde\assortment, i)
    % \condition j^* = j
    }
    =
    \sum_{j=0}^m
    q_j\expect[\tilde\assortment]{\choice(\tilde\assortment, i)
    \condition j^* = j}
    =
    \left(
    \sum_{j=\sigma(i)}^m q_j\right)\phi(\assortment,i)
    =
    p_i
\end{align*}
which completes the inductive step and finishes the proof.
\end{proof}



%In this section, we give the omitted proof
% in \Cref{sec:stochastic}.

% \begin{comment}
% \begin{numberedlemma}{\ref{lem:simplex in unit cube}}
% For any point $\mathbf p = (p_1, \dots, p_m) \in \R^m$
% s.t. $1\geq p_1 \geq \dots \geq p_m \geq 0$.
% Let $\mathbf p^{(j)}\in \R^m$ be the point where 
% the values of the first $j$ coordinates are 1,
% and the values of remaining coordinates are 0.
% Then,
% point $\mathbf p$ can be written as the convex combination of $m+1$
% points $\{\mathbf p^{(j)}\}_{j=0}^m$.
% \end{numberedlemma}
% \begin{proof}
% We prove the lemma by directly construct 
% the convex combination coefficients $\{q^{(j)}\}_{j=0}^m$ 
% as follows:
% $q^{(0)} = 1 - p_1$, $q^{(m)} = p_m$, 
% and $q^{(j)} = p_j - p_{j+1}$ for $j=1,\dots, m - 1$.
% \end{proof}

% \begin{numberedlemma}
% {\ref{lem:assortment polytope}}
% For any weak substitutable
% and downward-closed feasible choice model $\phi$,
% any assortment $\assortment, \assortmentspace$,
% and any target probability $\{p_i\}_{i\in \assortment}$
% such that $p_i \leq \choice(\assortment, i)$ for all $i\in \assortment$,
% Procedure~\ref{alg:sample assortment} 
% outputs an assortment $\assortment'$ at random and satisfies
% (i) $\assortment'\subseteq\assortment$; (ii)
% $\expect[\assortment']{\choice(\assortment', i)} = p_i$ 
% for all $i\in \assortment$.
% Moreover, it runs in time $\textrm{Poly}(n)$.
% \end{numberedlemma}
% \end{comment}

%\polytope*

% \begin{proof}{\textsl{Proof.}}
% To show the polynomial 
% running time,
% observe that 
% (a) the running time in each recursion
% is $\textrm{Poly}(n)$;
% and 
% (b) the number of recursion is 
% at most $|\assortment| \leq n$, 
% since $\assortment'$ called in the recursion
% satisfying that $|\assortment'| \leq |\assortment| - 1$.

% Property (i) holds by construction.
% We show property (ii) by induction on 
% $m = |\assortment|$,
% i.e., size of 
% assortment $\assortment$. 
% % Without loss of generality, we assume 
% % $\sigma(i) = i$ for all $i \in \assortment$.
% In this induction, 
% we use another simple property (iii)
% that
% $\phi(\assortment, i)\left(\sum_{j=\sigma(i)}^m q_j\right)  = p_{i}$
% for all $i\in \assortment$,
% which immediately hold by construction.

% \noindent\emph{Base Case ($m=1$).} 
% In this case
% Procedure~\ref{alg:sample assortment} randomly outputs
% $\emptyset$ or $\assortment$.
% By property (iii), the induction statement
% holds.

% \noindent\emph{Inductive step ($m > 1$).} 
% Fix an arbitrary product $i\in \assortment$.
% Notice that by construction
% $
% \expect[\tilde\assortment]{\choice(\tilde\assortment, i)
%     \condition j^* < \sigma(i)} = 0$,
% and 
% $
% \expect[\tilde\assortment]{\choice(\tilde\assortment, i)
%     \condition j^* = m}
%     =
%     \choice(\assortment, i)$.
% For any $j = i, \dots, m - 1$,
% and $\assortment' = \{\sigma(k)\}_{k=1}^{j}$. 
% Since the choice model $\choice$ is weak substitutable,
% i.e., $\choice(S', i) \geq \choice(S, i)$,
% invoking induction hypothesis on assortment $\assortment'$
% with $|\assortment'| \leq m-1$, we have 
%     $\expect[\tilde\assortment]{\choice(\tilde\assortment, i)
%     \condition j^* = j} = \choice(\assortment, i)$ for all $j = i, \dots, m - 1$.
%     Thus, invoking property (iii),
% \begin{align*}
% \expect[\tilde\assortment]{\choice(\tilde\assortment, i)
%     % \condition j^* = j
%     }
%     =
%     \sum_{j=0}^m
%     q_j\expect[\tilde\assortment]{\choice(\tilde\assortment, i)
%     \condition j^* = j}
%     =
%     \left(
%     \sum_{j=\sigma(i)}^m q_j\right)\phi(\assortment,i)
%     =
%     p_i
% \end{align*}
% which completes the inductive step and finishes the proof.
% \hfill\Halmos
% \end{proof}


==> tex/extra-EC.tex <==
We provide numerical justifications for the revenue performance of our proposed policies. By using a similar experimental setup to those in  \citet{GNR-14,RST-17}, we demonstrate their performance and compare them with other proposed policies in the literature, both when rental durations are infinite (no rental) or are finite and stochastic 
drawn from known distributions (with rentals). In a nutshell, we see considerable improvement in our revenue performance; see \Cref{sec:numerical} for details.


==> tex/figure-coupling.tex <==
\begin{tikzpicture}[scale = 0.5]

%short version

% \draw (0,0) rectangle (6,3) node[pos=.5] 
% {$\exanterev(\{\cumprice_i\}_{i=1}^n)$};

% \draw (0,8) rectangle (6,11) node[pos=.5]
% {$\pricerev(\{\cumprice_i\}_{i=1}^n)$};


% \draw (22,0) rectangle (28,3) node[pos=.5] 
% {$\exanterev(\{\revcurve_i\}_{i=1}^n)$};

% \draw (22,8) rectangle (28,11) node[pos=.5]
% {$\pricerev(\{\revcurve_i\}_{i=1}^n)$};


% \draw [vecArrow] (6.2, 1.5) -- (21.8, 1.5);
% \draw (14, 2.2) node {
	% [Thm.~\ref{thm:general EAR bound}] 
		% $\alpha\beta$-approx,};
% \draw (14, 0.8) node {if 
	% $\{\cumprice_i\}%_{i=1}^n
		% $ 
		% is downward $(\alpha,\beta)$-close to
		% $\{\revcurve_i\}%_{i=1}^n
		% $.};

% \draw [vecArrow] (6.2, 9.5) -- (21.8, 9.5);
% \draw (14, 10.2) node {
	% [Thm.~\ref{thm:general AP bound}]
		% $\alpha\beta$-approx,};

% \draw (14, 8.8) node {if 
	% $\{(\cumprice_i, \revcurve_i)\}$
		% is $(\alpha, \beta)$-regular.};


% \draw [vecArrow]  (3, 7.8) -- (3, 3.2);
% \draw (7.0, 6.0) node {
	% [Thm.~\ref{thm:linear bound}]
		% $\rho$-approx,};
% \draw (6.6, 5.0) node {if $\{\cumprice_i\}$
	% is concave.};

% \draw [vecArrow]  (25, 7.8) -- (25, 3.2);
% \draw (21.0, 6.0) node {
	% [Thm.~\ref{thm:linear bound}]
		% $\rho$-approx.};

% long version

\draw (10, 5) node {The $j^{\textrm{th}}$ unit of product $i$ under $\typesequence$};

\draw [vecArrow] (5, 1.5) -- (35, 1.5);
\draw (9, 2) -- (9, 1);
\draw (9, 0.5) node {$t_1$};
\draw (13, 2) -- (13, 1);
\draw (13, 0.5) node {$t_2$};
\draw (27, 2) -- (27, 1);
\draw (27, 0.5) node {$t_{k-1}$};
\draw (32, 2) -- (32, 1);
\draw (32, 0.5) node {$t_k$};
\draw (20, 2.5) node {$\dots\dots$}; 
\draw [fill=gray!0!white] (9, 3) rectangle (12, 1.57) node[pos=.5] {$d^{t_1}$};

\draw [fill=gray!25!white] (13, 3) rectangle (17, 1.57) node[pos=.5] {$d^{t_2}$};

\draw [fill=gray!75!white] (27, 3) rectangle (30, 1.57) node[pos=.5] {$d^{t_{k-1}}$};

\draw [fill=gray!100!white] (32, 3) rectangle (34, 1.57) node[pos=.5] {$d^{t_k}$};

	\draw (10, -1) node {The $j^{\textrm{th}}$ unit of product $i$ under $\inversetypesequence$};

\draw [vecArrow] (35, -4.5) -- (5, -4.5);
\draw (9, -4) -- (9, -5);
\draw (9, -5.5) node {$t_k'$};
\draw (13, -4) -- (13, -5);
\draw (13, -5.5) node {$t_{k - 1}'$};
\draw (27, -4) -- (27, -5);
\draw (27, -5.5) node {$t_2'$};
\draw (32, -4) -- (32, -5);
\draw (32, -5.5) node {$t_1'$};
\draw (20, -3.5) node {$\dots\dots$}; 
\draw [fill=gray!100!white] (9, -3) rectangle (7, -4.42) node[pos=.5] {$d^{t_k}$};

\draw [fill=gray!0!white] (13, -3) rectangle (10, -4.42) node[pos=.5] {$d^{t_1}$};

\draw [fill=gray!50!white] (27, -3) rectangle (23, -4.42) node[pos=.5] {$d^{t_{k-2}}$};

\draw [fill=gray!75!white] (32, -3) rectangle (29, -4.42) node[pos=.5] {$d^{t_{k-1}}$};


% \draw (0,0) rectangle (6,3) node[pos=.5] 
% {$\exanterev(\{\cumprice_i\}_{i=1}^n)$};

% \draw (0,8) rectangle (6,11) node[pos=.5]
% {$\pricerev(\{\cumprice_i\}_{i=1}^n)$};


% \draw (24,0) rectangle (30,3) node[pos=.5] 
% {$\exanterev(\{\revcurve_i\}_{i=1}^n)$};

% \draw (24,8) rectangle (30,11) node[pos=.5]
% {$\pricerev(\{\revcurve_i\}_{i=1}^n)$};


% \draw [vecArrow] (6.2, 1.5) -- (23.8, 1.5);
% \draw (15, 2.2) node {
	% Thm.~\ref{thm:general EAR bound}: 
		% $\zeta$-approx,};
% \draw (12.2, 0.8) node {if 
	% $\{\cumprice_i\}_{i=1}^n
		% $ 
		% is $\zeta$-close 
		% for ex ante };

% \draw (19.5, -0.2) node{
	% optimization to
		% $\{\revcurve_i\}_{i=1}^n
		% $.};

% \draw [vecArrow] (6.2, 9.5) -- (23.8, 9.5);
% \draw (15, 10.2) node {
	% Thm.~\ref{thm:general AP bound}:
		% $\alpha\beta$-approx,};

% \draw (11.7, 8.8) node {if 
	% $\{\cumprice_i\}_{i=1}^n
		% $ 
		% is $(\alpha,\beta)$-close 
		% for };

% \draw (19.5, 7.7) node{
	% price posting to
		% $\{\revcurve_i\}_{i=1}^n
		% $.};

% \draw [vecArrow]  (3, 7.8) -- (3, 3.2);
% \draw (7.0, 6.0) node {
	% Thm.~\ref{thm:linear bound}:
		% $\rho$-approx,};
% \draw (7.05, 5.0) node {if $\{\cumprice_i\}_{i=1}^n
	% $
		% is concave.};

% \draw [vecArrow]  (27, 7.8) -- (27, 3.2);
% \draw (23.0, 5.5) node {
	% Thm.~\ref{thm:linear bound}:
		% $\rho$-approx.};
\end{tikzpicture}




==> tex/literature-review.tex <==
\label{sec:furtherreview}
Assortment planning has an extensively growing 
literature over recent decades. We refer the reader to  related surveys and books \citep[cf.][]{KFV-08, lan-90, HT-98} for a comprehensive study.
\citet{VM-99} study the static model 
which captures the tradeoffs between
inventory costs and 
product variety under multi-nomial logit 
consumer choice model. 
Later works have 
considered various consumer choice models,
e.g., 
demand substitution model \citep{SA-00}, multinomial logit models
\citep{TV-04, GIPD-04, LV-08, top-13},
the Lancaster choice model
\citep{GH-06},
ranked-list preference 
\citep{HGS-10, GLS-16}, and non-parametric (data-driven)
choice model \citep{FJS-13}.

Real-time assortment has been studied massively more recently, both under the prior-free and Bayesian assumptions. For non-reusable products,
\citet{BKX-15} study a model with two products, i.i.d.\ consumer types and Poisson arrivals. \citet{CF-09} study a model with non-stationary consumer types and show $\tfrac{1}{2}$ performance guarantee
with respect to the clairvoyant benchmark. As discussed above, \citet{GNR-14} introduce inventory balancing algorithms and analyze their performance guarantee in prior-free setting. This analysis is later generalized and improved by \cite{MS-19} to the case where there are finite steps in the penalty function.


For real-time assortment of reusable products,
\citet{LR-10} study a model that assumes independent demands across products, without any choice behavior for the customers with infinite selling horizon. A follow up work from \citet{OS-18} extend this work to incorporate customer choice behavior and a finite selling horizon. \citet{CLS-17} study a model with multiple units of a single reusable product. They consider stochastic usage durations and advance reservations, and obtain data-dependent performance guarantees that are asymptotically optimal when the product inventory and the customer arrival rate scale up linearly at the same rate. Finally, \citet{RST-17} study Bayesian setting and \citet{GGISUW-19} study prior-free setting, as discussed in detail before. 

Recently, and after the online publication of an earlier version of this paper, we were informed of a forthcoming manuscript related to real-time assortment of reusable products in the prior-free setting by \citet{vineet-personal}. Based on private communications with authors and a  presentation at INFORMS 2019, we understand their work generalizes \citet{GGISUW-19} and gives an online policy with the asymptotic competitive ratio of $1-\frac{1}{e}$ when usage durations are drawn from a distribution that has a non-increasing probability distribution function in addition to some mass at infinity. Their algorithm and analysis is different from ours and their results diverge from ours in several ways. First, our paper focuses on a family of inventory balancing algorithms for a larger class of problems (including assortment with reusable resources). Second, we develop linear-programming based tools to compare our policies with the stronger offline LP benchmark (and not directly with the online clairvoyant policy). Finally, our $(1-\frac{1}{e})^2$-competitive algorithm for the stochastic scenario requires no distributional assumption, while the $(1 - \frac{1}{e})$-competitive algorithm aforementioned work requires the probability distribution function of return times to be non-increasing. 

%As discussed above, and show $\tfrac{1}{2}$ performance guarantee 
%with respect to optimal online dynamic programming;
%and a (inventory, fee)-dependent performance guarantee for non-reusable products.
%and show $\sfrac{1}{2}$ performance guarantee of greedy algorithm
%with respect to a clairvoyant benchmark.

For prior-free setting, our problem resembles some aspects of the online bipartite matching \citep[e.g.][]{KVV-90, BM-08, DJK-13} and the Adwards problem \citep[e.g.][]{MSVV-05, GM-08, GMNS-10, DHKMY-13}.
For Bayesian setting, our problem resembles some aspects of the prophet inequality matching \citep{AHL-12}, the Magician's problem \citep{ala-14}, and also the recenetly studied pricing with static calendar problem in \cite{MSZ-18} (which also studies static assortment policies without resubale resources). The techniques we use in the Bayesian scenario resemble the LP-method of \cite{A-07}, and also other methods for approximate dynamic programming (see \cite{SBAPW-04} for a comprehensive study). Another interesting related work to obtain improved (additive or regret-based) approximations for Bayesian online selection problem is \cite{VB-18}, which takes a different direction than our paper (although formally carrying over their techniques to the reusable resources problem is an interesting future direction).


==> tex/numerical-result.tex <==
To summarize our findings from the simulations of this section, we consider the two categories of scenarios mentioned above separately: 
\begin{enumerate}
\item{No rental setting} IB and all simulation-based algorithms 
have noticeably better performance 
than other algorithms.
Specifically, compare other algorithms with \texttt{Sim+OPTDis}
which guarantees the best theortical performance:
the average performance gap between \texttt{Sim+OPTDis}
and \texttt{GR} is 9.6\%,
the average performance gap between \texttt{Sim+OPTDis}
and \texttt{GR+APXLinValue} is 6.6\%,
the average performance gap between \texttt{Sim+OPTDis}
and \texttt{Rollout} is 7.1\%,
the average performance gap between \texttt{Sim+OPTDis}
and \texttt{IB} is 2.7\%.
{\color{red} Not sure if we should discuss the reason why \texttt{IB} 
performs better than \texttt{Rollout}, which contradicts the numerical
results in \citet{RST-17}. The main reason is that in their numerical experiment,
they recompute the estimators in \texttt{Rollout} after every 100 time 
periods which improves its performance.}
\end{enumerate}



Rental setting: \texttt{Sim+Infusion} and \texttt{Sim+MagicianDis}
performs noticeably better than other algorithms.
Specifically, for \texttt{Sim+Infusion} which guarantees the best
theoretical performance:
the average performance gap between \texttt{Sim+Infusion} and 
and \texttt{GR} is 3.6\%,
the average performance gap between \texttt{Sim+Infusion} and 
and \texttt{GR+APXLinValue} is 7.4\%,
the average performance gap between \texttt{Sim+Infusion} and 
and \texttt{Rollout} is 6.7\%,
the average performance gap between \texttt{Sim+Infusion} and 
and \texttt{IB} is 3.3\%. 
{\color{red} I'm curious why the expected revenue of \texttt{Expected-LP}
is not monotone in $\kappa$ for Table 4.}


==> tex/stochastic-exact-duration.tex <==
\label{sec:exact-duration}
In this section, we consider the setting where the platform  observes the (potential) rental duration for each product exactly once a consumer arrives. This feature, referred to as \emph{advanced reservation}, corresponds to online hospitality services such as Airbnb, where users report the duration of their stay to the platform before platform shows them a listing.


In our model, this is a special case where the rental duration distributions
encoded in consumer types are point mass. Hence, we can obtain the same competitive ratios against the offline LP benchmark $\EAR{\typedistributionsequence}$ in this setting as in \Cref{sec:stochastic-finite} by using \Cref{alg:SB} (for general rental time distributions), and as in
\Cref{sec:stochastic-infinite} by using \Cref{alg:SB infinite DP} and \Cref{alg:SB infinite magician} (for infinite rental times).



==> tex/stochastic-no-duration.tex <==
In this section, we consider the setting where the rental times are infinite, i.e., once products are purchased by consumers, they never return to the platform. In this setting, the inventory level of each product is weakly decreasing over time. This enables us to develop inventory-dependent discarding policies in polynomial time using dynamic programming. These discarding policies are more refined than the per-unit revenue thresholding policy discussed in \Cref{sec:stochastic-finite} and achieve a better competitive ratio  (i.e., $\infiniteboundtext$), which is near-optimal when inventories are large.
We propose two such policies: \emph{inventory-dependent revenue thresholds} (\Cref{sec:inventory-dep-simulation-based}) and \emph{discarding based on magician's advice} (\Cref{sec:inventory-dep-magician}).
The comparison between them is discussed in \Cref{sec:inventory-dep-comparison}.


\subsubsection{Inventory-dependent revenue thresholds by dynamic programming}
\label{sec:inventory-dep-simulation-based}

Fix a product $i\in [n]$. Similar to \Cref{sec:stochastic-finite-simple-DP},
we use dynamic programming  to
compute the expected revenue-to-go of the optimal discarding policy for this product that get suggestions from a simulation-based outer algorithm. This time, thanks to the monotonicity of inventory level of product $i$, the state of the aforementioned DP is one-dimensional and the expected revenue-to-go will only depend on the current inventory level. Therefore the DP is solvable, and thus its corresponding discarding rule is computable,  in polynomial-time


Specifically, let $\DP_{i, t}^I$ denote the expected revenue-to-go of product $i$ during $[t,T]$ from the optimal discarding policy, when $I$	is the remaining inventory at time $t$.
Similar to the discussion about the per-unit revenue
thresholds in \Cref{sec:stochastic-finite},
suppose assortment $\sampleassortment \sim \curexantetype$ is sampled 
at time $t$. If the DP discarding policy 
discards the product $i$ from the sampled assortment $\sampleassortment$,
the expected revenue-to-go becomes $\DP_{i, t + 1}^I$;
otherwise, with probability $\choice^{\type_t}(\sampleassortment, i)$ 
the consumer selects product $i$ and the expected revenue-to-go becomes
$\DP_{i,t + 1}^{I - 1} + \curreward$.
With the remaining probability, product $i$ is not selected and 
the expected revenue-to-go is $\DP_{i, t + 1}^I$.
Hence, we 
can calculate $\DP_{i, t}^I$ using dynamic programming (i.e., backward induction), with 
the following Bellman equation:
\begin{align}
	\label{eq:bellman equation infinite}
	\begin{split}
		&\DP_{i, t}^I = 
		%		\left(1 - 
		%		\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		%		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
		%		\curexantetype  
		%		\right)
		%		\DP_{i, t + 1}^I \\
		%		&\qquad+
		\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
		\curexantetype  
		\max\{\DP_{i, t + 1}^I,
			\curchoice
			(\curreward + 
			\DP_{i, t + 1}^{I - 1})
			+
			(1 - \curchoice)\DP_{i, t + 1}^I
		\},%\\
		%	&\text{and } 
		%	\DP_{i, T + 1}^I, \DP_{i, t}^0 = 0.
	\end{split}
\end{align}
After rearranging the terms, it is easy 
to observe that the final discarding rule will be an inventory-dependent revenue thresholding. Moreover, it will be
independent of $\{\curchoice\}$ as these terms cancel out:
\begin{align*}
	\left[\textrm{At time $t$ with type $\type_t$
			and inventory $I_i$, 
	$i\in \hat{\assortment}$ will be accepted}\right] 
	\Longleftrightarrow 
	\curreward    \geq 
	\DP_{i, t + 1}^{I_i}-\DP_{i, t + 1}^{I_i - 1}
\end{align*}

We are now ready to present our refined simulation-based policy using the above inventory-dependent revenue thresholds (\Cref{alg:SB infinite DP}).
\begin{algorithm}
	\caption{Simulation-based Algorithm with Inventory-dependent Revenue Thresholds}
	\label{alg:SB infinite DP}
	\begin{algorithmic}[1]
		\vspace{2mm}
		\State{Compute the optimal assignment of $\EAR{\typedistributionsequence}$ given the offline assortment oracle  (\Cref{asp:oracle}). Let  $\{\curalloctypeopt\}$ be the optimal assignment.} 

		\State{Set $\curexantetype\triangleq\curalloctypeopt\typedistribution_t(\type_t)$ for every $\assortment$,$t$ and $\type_t$ where optimal assignment has a non-zero entry.}	
		\State{Solve the dynamic programming with Bellman update described in \Cref{eq:bellman equation infinite} 
			and boundary condition $\DP_{i,T+1}^I, \DP_{i, t}^0 = 0$ for every product $i$ to obtain 
		$\{\DP_{i,t}^I\}_{i\in[n],t\in[\totaltime]}^{I \in [\inventory_i]}$.}
		%\State{Let $\curprice\triangleq \valueDPsimple_{i, t + 1}-\displaystyle\sum\nolimits_d\durationpdf_i^{\type_t}(d)\valueDPsimple_{i, t + d}$}, for all $i\in[n],t\in[\totaltime],\type_t\in\typespace_t$.
		\For{time $t=1$ to $T$}
		\State{Realize the consumer type $\type_t\in\typespace_t$.}
		\State {Sample $\hat{\assortment}\sim \{\curalloctypeopt\}_{\assortment\in\assortmentspace}.$}
		\For{products $i\in\hat{\assortment}$}
		\State{Let $I_i$ be the current inventory of product $i$.}
		\State{If $I_i = 0$ or 
			$ \curreward
			<
		\DP_{i, t + 1}^{I_i}-\DP_{i, t + 1}^{I_i - 1}$, remove $i$ from $\hat{\assortment}$.}
		\EndFor
		\State{Offer subset $\hat{\assortment}$ to the current consumer.}
		\EndFor
	\end{algorithmic}
\end{algorithm}


\begin{theorem}
	\label{thm:SB infinite DP}
	Let $\mininventory = \min_{i\in[n]}\inventory_i$ be the smallest inventory.
	The competitive ratio of \Cref{alg:SB infinite DP}
	against offline Bayesian expected LP benchmark, i.e., $\EAR{\typedistributionsequence}$
	is at least $\left(1-\tfrac{1}{\sqrt{\mininventory+3}}\right)$.
	Moreover, it runs in time
	$\textrm{Poly}(n,T, \sum_{t\in[\totaltime]}\lvert\typespace_t\rvert)$ given oracle access to an offline algorithm for assortment optimization (\Cref{asp:oracle}).
\end{theorem}

The proof of \Cref{thm:SB infinite DP} follows a similar structure
as for the per-unit revenue thresholds: (a) we first use induction to show 
$\{\DP_{i, t}^I\}$ are lower-bounds the for future revenue-to-go of \Cref{alg:SB infinite DP},
then (b) introduce a linear program to show $\DP_{i, 1}^{\inventory_i}$
is at least $1 - \sfrac{1}{\sqrt{\inventory_i + 3}}$ of the contribution
of product $i$ to the objective value of $\EAR{\typedistributionsequence}$.
For part (b), we use a technical lemma (\Cref{def:sand/barrier}, \Cref{lem:sand/barrier})
developed in
\citet{ala-14} described below.

\begin{definition}[Sand/Barrier Process, \citealp{ala-14}]
	\label{def:sand/barrier}
	Consider a tape of infinite length with one unit of infinitely divisible sand at position 
	0 and a barrier at position 1.
	A sequence of $q_1, \dots, q_\totaltime$ (with all $q_t \in [0, 1]$)
	and a parameter $\gamma \in (0, 1)$ are given as the input.
	The sand and the barrier are gradually moved to the right in $\totaltime$ rounds.
	At the $t$-th round the following takes place.
	The left most $\gamma$ fraction of the sand on the tape is selected and the
	$q_t$ fraction of this sand is moved one position to the right.
	This can be defined formally as follows.
	Let $s_t^j$ denote the amount of sand
	at postition $j$ at the beginning of round $t$
	and let $y_t^j\in[0, 1]$ denote the fraction of sand
	selected from position $j$ during round $t$.
	$y_t^j$ are chosen such that $\sum_i s_t^jy_t^j = \gamma$
	and such that for some integer $\theta_t$,
	$y_t^j = 1$ for any $j < \theta_t$,
	and $y_t^j = 0$  for any $j > \theta_t$.
	So during round $t$,
	a $q_ty_t^js_t^j$ amount of sand is moved from each position $j$ 
	to position $j + 1$.
	The barrier is moved one position to the right at the end
	of any round when the total amount of sand at the position
	of the barrier is more than $1- \gamma$.
	We will use $\lambda_t$ to denote the position of the barrier at the beginning of round $t$.
\end{definition}

\begin{lemma}[Sand/Barrier Process, \citealp{ala-14}]
	\label{lem:sand/barrier}
	For any $\gamma$ and
	any
	sequence $q_1, \dots, q_n$,
	throughout the sand/barrier process
	the position of the barrier 
	at the beginning of round $t$,
	i.e., $\lambda_t$,
	satisfies
	\begin{align*}
		\lambda_t \leq \sum_{\tpre = 1}^{t - 1}q_{\tpre}\gamma
		+\frac{1 - \gamma^{\lambda_t}}{1 - \gamma}.
	\end{align*}
\end{lemma}

\begin{proof}[Proof of \Cref{thm:SB infinite DP}]
	We first show for any product $i$, time $t$ and inventory $I$,
	the future expected revenue in \Cref{alg:SB infinite DP}
	from product $i$ with current inventory $I$ at time $t$ is
	at least $\DP_{i, t}^I$ by induction on time $t$ from $T + 1$ to 1.
	The base case $t = T + 1$ is satisfied due to our boundary assumption
	that $\DP_{i, T + 1}^I = 0$. 
	Now, suppose from time $t + 1$ to $T + 1$, the induction hypothesis holds.
	Consider the algorithm at time $t$.
	An assortment $\sampleassortment$ is sampled with probability $\curexantetype$.
	Let $\finalassortment \subseteq \sampleassortment$ be the assortment 
	offered to consumer at time $t$ after discarding.
	For any product $i$ with inventory $I$,
	the algorithm discards it if
	$\DP_{i, t + 1}^{I - 1} + \curreward < \DP_{i, t + 1}^{I}$.
	By induction hypothesis at time $t + 1$,
	it guarantees to gain future expected utility 
	at least $\max\{
		\DP_{i, t + 1}^I, 
		\choice^{\type_t}(\finalassortment, i)
		(\curreward + \DP_{i, t + 1}^{I - 1})
		+
		(1-\choice^{\type_t}(\finalassortment, i))
		\DP_{i, t + 1}^I, 
	\}$.
	Since the choice model satisfies substitutability (\Cref{asp:substitutability}),
	$\choice^{\type_t}(\sampleassortment, i) \leq 
	\choice^{\type_t}(\finalassortment, i)$ if $i \in \finalassortment$.
	Therefore, by similar calculations as in the proof of \Cref{lem:part-one-simple}, the induction hypothesis holds at time $t$, i.e.,
	$\DP_{i, t}^I$ lower-bounds the future expected revenue from product $i$ with inventory $I$ 
	at time $t$.
	Thus, the expected revenue of \Cref{alg:SB infinite DP} 
	from product $i$ from time $1$ is at least $\DP_{i, 1}^{\inventory_i}$.
	
	Next, we show  $\DP_{i, 1}^{\inventory_i}$ is at least $\left(1 - \tfrac{1}{\sqrt{\inventory_i + 3}}\right)$ fraction of the contribution of product $i$ to the objective value of $\EAR{\typedistributionsequence}$. In our analysis, we fix to an arbitrary product $i$, and normalize the contribution of product $i$ in $\EAR{\typedistributionsequence}$ to be $1$ without loss of generality. Based on the Bellman equation \eqref{eq:bellman equation infinite}, and normalized contribution in $\EAR{\typedistributionsequence}$, we can write the following program to lower-bound the value of $\DP_{i, 1}^{\inventory_i}$,
	\begin{align}
		\label{eq:infinite DP program}
		\begin{array}{llll}
			{\min
			\limits_{\mathbf \reward, \mathbf \DP \geq \mathbf 0}}~~&
				\DP_{i, 1}^{\inventory_i}
				&\text{s.t.}& \\[1em]
							&
				\DP_{i, t}^I \geq
				\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
				\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
				\curexantetype  
				\max\{\DP_{i, t + 1}^I, & & \\
																   &
				\qquad\qquad
				\curchoice
				(\curreward + 
				\DP_{i, t + 1}^{I - 1})
				+
				(1 - \curchoice)\DP_{i, t + 1}^I
			\}
			& t \in [\totaltime],\ I \in [\inventory_i]&
			\\[1em]
			&
			\displaystyle\sum\nolimits_{t=1}^{\totaltime}
			\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
			\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
			\curreward
			\curchoice
			\curexantetype
			\geq 1
			& &
		\end{array}
	\end{align}
	where the variables are $\{\curreward\}$ and $\{\DP_{i, t}^I\}$.
	To prove our result, it is sufficient to show that 
	for all inventory feasible $\{\curexantetype\}$, (i.e.\ 
	$\sum_{t, \type_t, S}\curexantetype\curchoice \leq \inventory_i$),
	the value of program \eqref{eq:infinite DP program} is 
	at least $1 - \tfrac{1}{\sqrt{\inventory_i + 3}}$.
	To see this, we relax the first constraint
	in \eqref{eq:infinite DP program} by 
	switching the outer summation and max operator,
	which provides 
	a relaxed linear program as follows,
	\begin{align*}
		\begin{array}{llll}
			{\min
			\limits_{\mathbf \reward, \mathbf \DP \geq \mathbf 0}}~~&
				\DP_{i, 1}^{\inventory_i}
				&\text{s.t.}& \\[1em]
							&
				\DP_{i, t}^I \geq
				\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
				\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
				\curexantetype  
				\curchoice
				(\curreward + 
				\DP_{i, t + 1}^{I - 1}) && \\
										& 
				\qquad\qquad+
				\left( 1 - 
					\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
					\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
					\curexantetype  
					\curchoice
				\right)
				\DP_{i, t + 1}^I
				& t \in [\totaltime],\ I \in [\inventory_i]&
				\langle\alpha_t^I\rangle
				\\[1em]
				&
				\DP_{i, t}^I \geq \DP_{i, t + 1}^I
				& t \in [\totaltime],\ I \in [\inventory_i]& 
				\langle\beta_t^I\rangle
				\\[1em]
				&
				\displaystyle\sum\nolimits_{t=1}^{\totaltime}
				\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
				\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
				\curreward
				\curchoice
				\curexantetype
				\geq 1
				& & 
				\langle\mu\rangle
			\end{array}
		\end{align*}
		We write its dual program with dual variable $\alpha_t^I$, $\beta_t^I$ and 
		$\gamma$ as follows
	\begin{align*}
		\begin{array}{llll}
			{\max
			\limits_{\boldsymbol{\alpha, \beta, \mu} \geq \mathbf 0}}~~&
				\mu
				&\text{s.t.}& \\[1em]
				& \alpha_1^{\inventory_i} + \beta_1^{\inventory_i} \leq 1
				& & \langle\DP_{i, 1}^{\inventory_i}\rangle 
				\\[1em]
				& \alpha_1^{I} + \beta_1^{I} \leq 0
				& I \in [\inventory_i - 1]& \langle\DP_{i, 1}^{I}\rangle 
				\\[1em]
							&
				\alpha_{t + 1}^{I} + \beta_{t + 1}^I \leq
				\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
				\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
				\curexantetype  
				\curchoice
				\alpha_{t}^{I + 1}
				+
				&& \\
										& 
				\qquad\qquad+
				\left( 1 - 
					\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
					\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
					\curexantetype  
					\curchoice
				\right)
				\alpha_{t}^I + \beta_{t}^I
				& t \in [\totaltime - 1],\ I \in [\inventory_i]&
				\langle\DP_{i, t+ 1}^I\rangle
				\\[1em]
				&
				\displaystyle\sum\nolimits_{t=1}^{\totaltime}
				\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
				\curchoice
				\curexantetype 
				\mu & & \\
					   &
				\qquad\qquad
				\leq 
				\displaystyle\sum\nolimits_{t=1}^{\totaltime}
				\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
				\left(
				\curchoice
				\curexantetype
				\left(
				\displaystyle\sum\nolimits_{I = 1}^{\inventory_i}
		\alpha_t^I \right)\right)
				& \type_t \in \typespace& 
				\langle \curreward\rangle
			\end{array}
		\end{align*}
		By weak duality, any feasible dual solution offers 
		a lower bound for the primal. 
		
		
Now, suppose we are interested in generating a feasible dual assignment where the all the constraints corresponding to $\{\DP_{i, t}^I\}_{I\in[\inventory_i,t\in[T]}$ in the above dual program are tight. Let : $$q_t \triangleq \sum_{\type_t\in \typespace_t}\sum_{\assortment\in\assortmentspace}\curexantetype\curchoice$$
 Note that we need to have:
\begin{equation}
\label{eq:sand-initial}
\alpha_1^{\inventory_i} + \beta_1^{\inventory_i} = 1~~~~~~~,~~~~~~~ \alpha_1^{I} + \beta_1^I=0,~I\neq \inventory_i~,
\end{equation}
and for all $t\in[1:T-1], I\in[1:\inventory_i]$ we need to have:
\begin{equation}
\label{eq:sand-dynamic}
\alpha_{t + 1}^{I} + \beta_{t + 1}^I =q_t\alpha_{t}^{I + 1} +\left(1 - q_t\right)\alpha_{t}^I + \beta_{t}^I
\end{equation}
We now construct such a feasible dual solution by using the sand/barrier argument (\Cref{def:sand/barrier} and \Cref{lem:sand/barrier}). Let $\{s_t^j\}, \{y_t^j\}$, and $\{\lambda_t\}$ be variables defined in sand/barrier process of \Cref{def:sand/barrier}, with parameter $T$, $\{q_t\}_{t\in[T]}$ and $\gamma = 1 - \tfrac{1}{\sqrt{\inventory_i+3}}$. Think of different inventory levels as different positions on the tape of sands, but in reveres order. In other words, position $\inventory_i -I$ corresponds to inventory level $I$ (basically, sand moves from higher to lower inventory levels). We have $T$ number of rounds of sand/barrier process.  At round $t$ of the process, there is a total of $s_t^{\inventory_i-I}$ unit of sand at each position $\inventory_i-I$ for $I\in[\inventory_i]$. The amount of sand $s_t^{\inventory_i-I}$ is divided into selected sand $ s_t^{\inventory_i - I}y_t^{\inventory_i - I}$ that determines $\alpha_t^I$, and non-selected sand $s_t^{\inventory_i - I}(1 - y_t^{\inventory_i - I})$, that determines $\beta_t^I$. In summary, we construct the dual solution as follows,
		\begin{align*}
			\mu = \gamma,%1 - \frac{1}{\sqrt{\inventory_i + 3}},
			\;\;
			\alpha_t^{I} = s_t^{\inventory_i - I}y_t^{\inventory_i - I},
			\;\;
			\mbox{and}
			\;\;
			\beta_t^{I} = s_t^{\inventory_i - I}(1 - y_t^{\inventory_i - I}).
		\end{align*}
		
Note that \cref{eq:sand-initial} is satisfied by above dual construction, as there is one unit of sand at position $0$ of the tape (corresponding to inventory level $\inventory_i$) at time $t=1$, and no other sand exists on the tape at this time. Moreover, \cref{eq:sand-dynamic} is satisfied because of the dynamic of the sand/barrier process: from time $t$ to $t+1$, $q_t$ fraction of selected sand at each position $\inventory_i-I-1$ (which amounts to $q_t\alpha_{t}^{I + 1}$) moves to the position $\inventory_i-I$, and only $1-q_t$ fraction of the selected sand at position $\inventory_i-I$ (which amounts to $\left(1 - q_t\right)\alpha_{t}^I$) remains unmoved. Note that there always exists a total of $\gamma=\mu$ unit of selected sand, hence $\sum_{I=1}^{\inventory_i}\alpha_t^I=\gamma=\mu$. This ensures that constraints of the dual corresponding to $\{\curreward\}$ are satisfied.  Finally, based on the description of sand/barrier process in \Cref{def:sand/barrier}, only $\inventory_i$ positions of tape will have sand (and hence this dual construction is well-defined) if the barrier never passes position $\inventory_i$, i.e., $\lambda_{T + 1} \leq \inventory_i$.
		Invoking \Cref{lem:sand/barrier} and rearranging the terms
%		\begin{align*}
%			\lambda
%		\end{align*}
%		which 
		finish the proof.
	\end{proof}

	\begin{remark}
	In the proof of \Cref{thm:SB infinite DP}, 
	we introduced a relaxation from program \eqref{eq:infinite DP program} 
	by swapping the summation and maximum. This relaxation 
	is indeed not a strict relaxation, 
	since it is without loss of generality to 
	consider an instance which
	compresses all $\type_t\in \typespace_t$ into a single type $\hat\type_t$
	as follows:
	a deterministic type 
	$\hat{\type}_t$ appears at time $t$;
	$\hat X_{S, t, \hat\type_t} = \sum_{\type_t \in \typespace_t}
	\sum_{\assortment\in\assortmentspace}\curchoice\curexantetype$
	if $S = \{i\}$ and 0 otherwise;
	$\hat\reward_i^{\hat\type_t} = \frac{\sum_{\type_t \in \typespace_t}
			\sum_{\assortment\in\assortmentspace}\curreward\curchoice\curexantetype
	}{
	\hat X_{\{i\}, t, \hat\type_t}}$.
	\end{remark}

	\subsubsection{Inventory-dependent discarding by the ``Magician's Problem''}
	\label{sec:inventory-dep-magician}
	Our second discarding policy starts with a simple discarding idea as follows. Once an assortment $\sampleassortment \sim \curexantetype$ is sampled by the simulation outer algorithm, we discard each product independently with probability $\tfrac{1}{2}$. We also discard products whose inventories are exhausted to ensure feasibility. Now consider any time $t$ and fix a product $i$. Since assignment $\{\curexantetype\}$ satisfies the inventory constraint of product $i$ in expectation, by Markov inequality, the simulation-based algorithm that independently discards each product with probability $\tfrac{1}{2}$ has not yet exhausted the inventory of product $i$ with probability at least $\tfrac{1}{2}$ at this time. As this policy discards the product $i$ with probability $\tfrac{1}{2}$, no matter what set $\sampleassortment$ is sampled, it only gets $\tfrac{1}{4}$ fraction of the contribution of this product in the expected LP objective in expectation. Therefore, the resulting policy is $\tfrac{1}{4}$-competitive against the offline expected LP benchmark.
	
	To achieve a better competitive ratio, notice that if a simulation-based algorithm satisfies (a) inventory feasibility and (b) independently discards each product $i$ at each time with probability at most $\gamma$
	regardless of sampled assortments $\sampleassortment$ and consumer types $\type_t$, its competitive ratio is at least $\gamma$. This problem of minimizing the maximum discarding probability to guarantee inventory feasibility has been studied in \citet{ala-14} as the {Magician's Problem}. We sketch its definition and its corresponding algorithmic consequence below. For more details, see \citet{ala-14}.

	\begin{definition}[The Magician's Problem, \citealp{ala-14}]
		A magician is presented with a sequence of boxes one by
		one in an online fashion. There is a prize hidden in one of the boxes.
		The magician has $\inventory$
		magic wands that can be used to open the boxes.
		If a wand is used on box $t$,
		it opens, 
		but with a probability $x_t$,
		which is written on the box, the wand breaks.
		The magician wishes to maximize the probability of obtaining the prize,
		but unfortunately the sequence of boxes, the written probabilities,
		and the box in which the prize is hidden are arranged by a villain,
		and the magician has no prior information about them (not even the number of boxes).
		However, it is guaranteed that
		$\sum_t x_t \leq \inventory$,
		and that the villain has to prepare the sequence of boxes in advance (i.e.,
		cannot make any changes
		once the process has started).
	\end{definition}

	In the language of assortment optimization, for an arbitrary product $i$, 
	it can be thought as an instance of the Magician's Problem, where $\inventory_i$ wands correspond $\inventory_i$ initial inventory,
	opening box $t$ corresponds to do not discard this product at time $t$,
	and written probability $x_t$ 
	corresponds to $\sum_{\type_t\in\typespace_t}\sum_{\assortment\in\assortmentspace}
		\curexantetype\curchoice$.
	\citet{ala-14} proposed and analyzed the following algorithm which guarantees
	to open each box with probability at least $1 - \sfrac{1}{\sqrt{\inventory + 3}}$
	(for $\inventory$ wands).

	\begin{definition}[$\gamma$-Conservative Magician, \citealp{ala-14}]
		\label{def:conservative magician}
		The magician adaptively computes a sequence of 
		(inventory) thresholds $\hat I_1, \hat I_2, \dots \in \Z_+$
		and makes a decision about each box as follows:
		let $I_t$ denote the number of unbroken wands 
		prior to seeing the $t$-th box;
		the magician makes a decision about box $t$
		by comparing $I_t$ against $\hat I_t$;
		if $I_t > \hat I_t$,
		it opens the box;
		if $I_t < \hat I_t$,
		it does not open the box;
		and if $I_t = \hat I_t$,
		it uses randomness and opens 
		the box with some probability (defined below).
		The magician chooses the largest threshold
		$\hat I_t$ for which $\prob{I_t \geq \hat I_t} \geq \gamma$
		where the probability is computed ex ante (i.e.,
		not conditioned on past broken wands).
		Let $\inventorycdfi_t^I \triangleq \prob{I_t \geq I}$
		be the probability that there is at least $I$ unbroken
		wands prior to seeing box $t$.
		Let $\magicprob_t^I$ be the probability that  
		the magician chooses to \emph{discard} (i.e., do not open) box $t$ when 
		there is $I$ unbroken wands at that moment,
		which is defined formally as follows,
		\begin{align}
			\label{eq:magician prob}
			%\prob{S_t = 1\condition I_t} 
			\magicprob_t^I
			&=
			\begin{cases}
				    0, & I > \hat I_t \\
				1 - \sfrac{(\gamma - \inventorycdfi_t^{\hat I_t + 1})}
				{(
					\inventorycdfi_t^{\hat I_t}
					-
					\inventorycdfi_t^{\hat I_t  + 1}
				)}, & I = \hat I_t\\
				    1, & I < \hat I_t
				  \end{cases} \\
				  \nonumber
				  \hat I_t &= \max\{I \condition \inventorycdfi_t^I \geq \gamma\}
			  \end{align}
			where $\inventorycdfi_{t + 1}$ can 
			be computed from $\inventorycdfi_t$ and $x_t$
			as follows,
		%	by the following Bellman update equation,
			\begin{align}
				  \nonumber
		\inventorycdfi_{t + 1}^I &= 
		\begin{cases}
			(1 - \magicprob_t^{I + 1}) x_t (\inventorycdfi_t^{I + 1} - \inventorycdfi_t^{I}) + 
			(1 - (1 - \magicprob_t^I)x_t)(\inventorycdfi_t^{I} - \inventorycdfi_t^{I - 1}) +
			\inventorycdfi_{t + 1}^{I + 1},
			& t \geq 1,\ 0 \leq I \leq c \\
			1, & t = 0,\ 0 \leq I \leq c \\
			0, & \text{otherwise}
		\end{cases}
		%\intertext{
		%	where $s_t^I = \prob{S_t = 1\condition I_t = I}$.
		%}
		\end{align}
	\end{definition}

	
	\begin{lemma}[$\gamma$-Conservative Magician, \citealp{ala-14}]
		\label{lem:conservative magician}
		For any $\gamma \leq 1 - \sfrac{1}{\sqrt{\inventory + 3}}$,
		a $\gamma$-conservative magician with $\inventory$ wands opens 
		each box with an ex ante probability at least $\gamma$.
	\end{lemma}

	Thus, with $\gamma$-conservative magician, we can design the 
	simulation-based algorithm as follows.

\begin{algorithm}
	\caption{Simulation-based Algorithm with Conservative Magician}
	\label{alg:SB infinite magician}
	\begin{algorithmic}[1]
		\vspace{2mm}
		\State{Compute the optimal assignment of $\EAR{\typedistributionsequence}$ given the offline assortment oracle  (\Cref{asp:oracle}). Let  $\{\curalloctypeopt\}$ be the optimal assignment.} 

		\State{Set $\curexantetype\triangleq\curalloctypeopt\typedistribution_t(\type_t)$ for every $\assortment$,$t$ and $\type_t$ where optimal assignment has a non-zero entry.}	
		\State{Set $\{\magicprob_{i, t}^I\}$ be the probability 
			defined 
			in $(1 - \sfrac{1}{\sqrt{\inventory_i + 3}})$-conservative magician
		(\Cref{def:conservative magician}) for each product $i$.}
	%	\State{Set $\{\hat I_{i, t}\}$ be the thresholds 
	%		in $(1 - \sfrac{1}{\sqrt{\inventory_i + 3}})$-conservative magician
	%		(\Cref{def:conservative magician}) for each product $i$.
	%}
		\For{time $t=1$ to $T$}
		\State{Realize the consumer type $\type_t\in\typespace_t$.}
		\State {Sample $\hat{\assortment}\sim \{\curalloctypeopt\}_{\assortment\in\assortmentspace}.$}
		\For{products $i\in\hat{\assortment}$}
		\State{Let $I_i$ be the current inventory of product $i$.}
		\State{Remove $i$ from $\hat{\assortment}$ 
			with probability $\magicprob_{i, t}^{I_i}$.
	}
		\EndFor
		\State{Offer subset $\hat{\assortment}$ to the current consumer.}
		\EndFor
	\end{algorithmic}
\end{algorithm}


\begin{theorem}
	\label{thm:SB infinite magician}
	Let $\mininventory = \min_{i\in[n]}\inventory_i$ be the smallest inventory.
	The competitive ratio of \Cref{alg:SB infinite magician}
	against offline expected benchmark, i.e., $\EAR{\typedistributionsequence}$
	is at least $(\infiniteboundtext)$-competitive.
	Moreover, it runs in time
	$\textrm{Poly}(n,T, \sum_{t\in[\totaltime]}\lvert\typespace_t\rvert)$ given oracle access to an offline algorithm for assortment optimization (\Cref{asp:oracle}).
\end{theorem}
\begin{proof}
	By \Cref{lem:conservative magician},  \Cref{alg:SB infinite magician} discards each product from the sampled assortment with probability 
	at most $\sfrac{1}{\sqrt{\mininventory + 3}}$, 
	regardless of consumer types or sampled assortment.
	Hence, it is $(\infiniteboundtext)$-competitive.
\end{proof}

\subsubsection{Comparison}
\label{sec:inventory-dep-comparison}
Even though \Cref{alg:SB infinite DP} and \Cref{alg:SB infinite magician}
have the same competitive ratios, their performance might be different over stochastic instances in various applications. Generally speaking, since \Cref{alg:SB infinite DP} makes the discarding decision 
based on the realized consumer types while \Cref{alg:SB infinite magician} does not utilize this information,
we expect that the former algorithm achieves higher revenue than the latter algorithm
if consumer types in each time period
are truly random (i.e., non deterministic).\footnote{As discussed above, the competitive ratio of 
	\Cref{alg:SB infinite DP} is achieved in an instance when consumer types at each time period are deterministic.}
On the other hand, \Cref{alg:SB infinite DP} 
requires a backward dynamic programming while 
\Cref{alg:SB infinite magician} only requires a forward dynamic programming,
which makes the latter algorithm faster in practice and its implementation requires less memory (as one only needs to compute DP entries corresponding to observed inventory levels and not all inventory levels).


==> tex/stochastic.tex <==

\label{sec:stochastic}
In several applications of assortment planning, specially in web-based domains, the platform has a considerable amount of prior knowledge about its consumers. This prior knowledge is either due to market research on types of consumers of the platform, or due to statistical study of the previous interactions of the same consumers with the platform. The Bayesian approach to model such settings is to describe platform's prior knowledge about the consumers as known distributions over types. Following this approach,  we study the real-time assortment optimization when types are independent across time and realized in an online fashion from known distributions $\typedistributionsequence$. A similar model has been studied in~\citep{RST-17}. We consider both finite (\Cref{sec:stochastic-finite}) and infinite (\Cref{sec:stochastic-infinite}) stochastic rental times. 

From a technical point of view, an important distinction between Bayesian and prior-free settings is that in the Bayesian setting nothing about the input instance is information theoretically hidden from an online algorithm for this problem. In fact, this problem is an stochastic online optimization. For such a problem, designing an online algorithm to maximize expected revenue given the prior information is purely computational and can be done using prohibitively expensive dynamic programming. Notably, this computational task is a special case of optimal online policy design for Markov Decisions Processes (MDP), which is P-SPACE hard~\citep{PT-1987}\footnote{We should also assert, to the best of our knowledge no formal argument exists in the literature for showing any computational hardness result for the special case of online stochastic assortment optimization (or even online stochastic matching).}. While it is unlikely to be able to directly solve for the dynamic programming solution, we can still try to get leverage from the prior information about heterogeneous time-varying consumers to design polynomial time policies.

Building intuitions based on the above observation leads us to the first main technical ingredient of our algorithms in this section. In particular, we show the expected LP benchmark proposed in \Cref{sec:prelim} ($\EAR{\typedistributionsequence}$) can be solved efficiently given access to an oracle algorithm for the offline assortment optimization problem. This is in contrast to possibility of solving the expected LP benchmark in the prior-free setting, as no online algorithm has  information about future types and hence cannot compute this benchmark.

After solving the LP, we use the optimal assignment in a modular way to design \emph{simulation-based} online algorithms that achieve (optimal) constant competitive ratios for this problem against the offline Bayesian expected LP benchmark. At high level, a simulation-based algorithm follows the optimal assignment of the expected LP by first picking a subset drawn from a probability distribution equal to the current expected LP optimal assignment. It then discard some of the products in this suggested set in a systematic way to (1) maintain inventory feasibility, and (2) to not lose a lot of revenue in expectation.

\subsection{Solving the Bayesian Expected LP}
\label{sec:stochastic-lp-solving}
We first sketch a technical lemma (see \cite{GLS-1981} for a detailed proof).
\begin{lemma}
\label{lem:ellipsoid-dual}
Suppose a primal linear program is bounded and feasible. Moreover, suppose its dual has a separation oracle with running time at most $\tau$. Then primal admits an optimal solution that has $\textrm{Poly}(\tau,m)$ non-zero entries and can be computed in $\textrm{Poly}(\tau,m)$ time, where $m$ is the number of dual variables (primal constraints). 
\end{lemma}
\begin{proof}[Proof sketch.]
Because primal LP is feasible and bounded, dual is also feasible and bounded. Now consider running ellipsoid algorithm with the separation oracle to solve the dual. Ellipsoid can solve the dual in $\textrm{Poly}(\tau,m)$ time. Now by looking at the run of ellipsoid and considering only dual constraints that ellipsoid returns as violated,  we can find $\textrm{Poly}(\tau,m)$ many constraints in the dual such that the dual value does not change if we throw away the remaining constraints. Note that constraints in the dual correspond to variables in the primal. So, we can throw away all the variables in the primal except the ones corresponding to the constraints in the dual that the separation oracles asks us to keep, and the LP value does not change. Now we have a compact LP in the primal, which we can again solve to get the succinct primal solution with $\textrm{Poly}(\tau,m)$ non-zero entries and in time $\textrm{Poly}(\tau,m)$.
\end{proof}
We are now ready to show that expected LP can be solved efficiently by the offline oracle.
\begin{proposition} Given an algorithm for offline assortment (\Cref{asp:oracle}), an optimal assignment $\{\curalloctypeopt\}$ of~$\EAR{\typedistributionsequence}$ can be computed efficiently in time $\textrm{Poly}(n,T, \sum_{t\in[\totaltime]}\lvert\typespace_t\rvert)$. Moreover, $\{\curalloctypeopt\}$ has no more than $\textrm{Poly}(n,T, \sum_{t\in[\totaltime]}\lvert\typespace_t\rvert)$ non-zero entries.  
\end{proposition}

\begin{proof}  $\EAR{\typedistributionsequence}$ is an LP with exponentially many variables and $(nT+T)$ constraints. Hence its dual has only $(nT+T)$ variables and exponentially many constraints. Here is the dual LP, with dual variable $\inventorydual$ 
	and $\probdual$:
\begin{align*}
	\begin{array}{rlll}
		\min
		\limits_{\boldsymbol{\theta},\boldsymbol{\lambda} \geq \mathbf 0} &
		\displaystyle\sum\nolimits_{t=1}^\totaltime
		\displaystyle\sum\nolimits_{i=1}^n
		\inventory_i\inventorydual+ \displaystyle\sum\nolimits_{t =1}^\totaltime\sum\nolimits_{\type_t\in\typespace_t}\probdualtype & \text{s.t.} &\\[1em]
		&
		\probdualtype + \displaystyle\sum\nolimits_{i = 1}^n\displaystyle\sum\nolimits_{\tpre= t}^T\typedistribution_t(\type_t)\durationcdfi^{\type_t}_i(\tpre-t)\curchoice\theta_{i,\tpre}\geq \displaystyle\sum\nolimits_{i = 1}^n
		\curreward \typedistribution_t(\type_t)\curchoice
		& \assortment \in \assortmentspace,\ t \in [\totaltime],\type_t\in\typespace_t
		%\forall i\in[n],t \in [T] 
		&
	\end{array}
\end{align*}	

Now, fix $t\in[\totaltime], \type_t\in\typespace_t$, and consider the group of dual constraints corresponding to $t$ and $\type_t$. In order to obtain a separation oracle for this group of constraints, given $\probdualtype$ and $\{\theta_{i,\tpre}\}$ one needs to find a set $\hat{S}\in\underset{\assortment\in\assortmentspace}\argmax~{\displaystyle\sum\nolimits_{i=1}^n\hat{R}_i\choice^{\type_{t}}(\assortment,i)}$, where
\begin{equation*}
\hat{R}_i\triangleq\typedistribution_t(\type_t)\left(\curreward-\displaystyle\sum\nolimits_{\tpre= t}^T\durationcdfi^{\type_t}_i(\tpre-t)\theta_{i,\tpre}\right)
\end{equation*}
Then if $\probdualtype\geq \displaystyle\sum\nolimits_{i=1}^n\hat{R}_i\choice^{\type_{t}}(\hat\assortment,i)$ these constraints are satisfied and if not the constraint corresponding to $t,\type_t,\hat{\assortment}$ is a separating hyperplane.  Note that because of downward-closeness of $\assortmentspace$, i.e., \Cref{asp:down-closed}, and weak-substitutability of $\curchoice$, i.e., \Cref{asp:substitutability}, we can discard products for which $\hat{R}_i<0$, and hence without loss of generality assume $\hat{R}_i\geq 0$. Therefore, thanks to \Cref{asp:oracle}, one can find such a subset $\hat \assortment$ with one call to the oracle. By a polynomial time search over all possible $t$ and $\type_t$, dual will have a separation oracle with running time $\textrm{Poly}(n,T,\sum_{t\in[\totaltime}\lvert\typespace_t\rvert)$. Invoking \Cref{lem:ellipsoid-dual} finishes the proof.
\end{proof}


% \subsection{Simulation-based Policy for General Rental Distributions
% and Large Inventory}
% \input{FNS/tex/bayesian-large-inventory}

\subsection{Simulation-based Policy for General Rental Distributions}
\label{sec:stochastic-finite}
In this section, we propose and analyze our first simulation-based policy.  Suppose $\{\curalloctypeopt\}$ be the optimal assignment of $\EAR{\typedistributionsequence}$. As $\emptyset\in\assortment$,  w.l.o.g. we can assume there always exists an optimal assignment where:
\begin{equation*}
\displaystyle\sum\nolimits_{\assortment\in \assortmentspace}\curalloctypeopt= 1~~~~~~\forall t \in [\totaltime],\ \type_t\in\typespace_t
\end{equation*}
Now,  the main idea is to do the assortment in two steps at each time $t$:
\begin{enumerate}[label=(\roman*)]
\item Upon realizing type $\type_t$ at time $t$, an outer procedure \emph{suggests} $\hat{\assortment}\sim \{\curalloctypeopt\}_{\assortment\in\assortmentspace}$ to be assorted, i.e., samples $\hat{\assortment}$ from the probability distribution $\{\curalloctypeopt\}_{\assortment\in\assortmentspace}$ over $\assortmentspace$,
\item For each product $i\in\hat{\assortment}$, a separate inner discarding procedure decides whether to put this product in the final assortment or not. If no units of product $i$ is available on-hand, it will be discarded to guarantee inventory feasibility. Otherwise, it will only be selected in the final assortment if $\curreward\geq \curprice$, where $\curprice$ are static \emph{per-unit revenue thresholds} computed by the algorithm up-front (will be discussed later).
\end{enumerate}
Step (\rom{1}) is a loss-less randomized rounding for optimal solution of the expected LP benchmark $\EAR{\typedistributionsequence}$; however this randomized assortment only guarantees inventory feasibility of each product in expectation. The role of step (\rom{2}) is to not only guarantee inventory feasibility for every sample path of the history, but also to guarantee only products with high per-unit revenue are assorted.

 Technically speaking, for each product $i$ one can consider a separate dynamic programming formulation to optimally make discarding decisions. This formulation will maximize per-unit revenue-to-go of assorted units of product $i$ over the time finite horizon $[1:T]$,  given the randomized suggestion of step (\rom{1}). The drawback is this approach requires a high-dimensional state variable that keeps track of the on-hand product inventories, as well the inventory of units of the product that are in use (and will return to inventory at different times). A major ingredient of our algorithm is to replace this high-dimensional dynamic programming with a simple one that is \emph{inventory independent}, and uses a pessimistic upper-bound of $\inventory_i$ on the actual inventory in the Bellman equation for updating optimal per-unit revenue-to-go of product $i$.
 
 
 \subsubsection{Dynamic Programming for Per-unit Revenue-to-go with Replenishment.} 
 \label{sec:stochastic-finite-simple-DP}
In the rest of this section, let $\curexantetype\triangleq\curalloctypeopt\typedistribution_t(\type_t)$ for every $\assortment$,$t$ and $\type_t$. Suppose at each time $t$ a randomized subset $\hat{S}\sim\curexantetype$ is sampled (as the outer procedure samples independently from $\type_t\sim \typedistribution_t$). Fix a product $i\in[n]$, with initial inventory of $\inventory_i$ units. Now, consider a hypothetical scenario where an exogenous process \emph{replenishes the inventory} at each time to guarantee we always have $\inventory_i$ units of the product on-hand, no matter how many units are currently under rental. In this new problem, the goal is to design an online policy to discard or accept units of the product upon suggestion of the outer algorithm, in order to maximize per-unit revenue-to-go.
 
 We can formulate the above problem using a simple dynamic programming, where $\valueDPsimple_{i,t}$ is the optimal per-unit revenue-to-go during time interval $[t:T]$. As a convention, let $\valueDPsimple_{i,T+1}=0$. To write the Bellman update equation of this DP at time $t$ using backward induction, suppose type $\type_t$ is realized and $\hat{\assortment}=\assortment$ (which happens w.p. $\curexantetype$). If optimal policy decides to discard product $i$, then per-unit revenue-to-go will be $\valueDPsimple_{i, t + 1}$. If optimal policy decides to not discard $i$, then w.p. $(1-\curchoice)$ the per-unit revenue-to-go will still be  $\valueDPsimple_{i, t + 1}$. However, w.p. $\curchoice$ consumer rents one of the $\inventory_i$ units (remember that inventory will always be full), and therefore generates a total revenue-to-go of $(\inventory_i-1)\valueDPsimple_{i, t + 1}$ (i.e., due to contribution of units not rented at time $t$; these units will transfer to the inventory at time $t+1$) plus $\curreward+\valueDPsimple_{i, t + d}$ upon realization of rental time $d\sim\durationpdf^{\type_t}_i$ (i.e., due to contribution of the rented unit). To summarize, we will have the following Bellman update equation:
 
%\begin{align}
%		\label{eq:bellman-equation-finite}
%		\begin{split}
%			&\valueDPsimple_{i,t}= 
%		\left(1 - 
%		\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
%		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}\curexantetype  \right)
%		\valueDPsimple_{i, t + 1}+\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
%		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
%		\curexantetype \\
%& 
%		\times\max\left\{\valueDPsimple_{i, t + 1}~,~\left(1 - \curchoice\right)\valueDPsimple_{i, t + 1}+ \curchoice\left(\frac{1}{\inventory_i}\sum_d\durationpdf^{\type_t}_i(d)\left(\curreward+\valueDPsimple_{i, t + d}\right)+\frac{\inventory_i-1}{\inventory_i}\valueDPsimple_{i, t + 1}\right )\right\}
%	\end{split}
%	\end{align}

\begin{align}
		\label{eq:bellman-equation-finite}
		\begin{split}
			&\valueDPsimple_{i,t}= \displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
		\curexantetype \\
& 
		\times\max\left\{\valueDPsimple_{i, t + 1}~,~\left(1 - \curchoice\right)\valueDPsimple_{i, t + 1}+ \curchoice\left(\frac{1}{\inventory_i}\sum\nolimits_d\durationpdf_i^{\type_t}(d)\left(\curreward+\valueDPsimple_{i, t + d}\right)+\frac{\inventory_i-1}{\inventory_i}\valueDPsimple_{i, t + 1}\right )\right\}
	\end{split}
	\end{align}

Note the update rule of the above dynamic programming can be simplified by rearranging the terms; Interestingly, the rule will be independent of $\inventory_i$ and $\curchoice$ as they cancel out: 
\begin{equation}
\left[\textrm{At time $t$ with type $\type_t$, $i\in \hat{\assortment}$ will be accepted}\right] \Longleftrightarrow \curreward \geq \valueDPsimple_{i, t + 1}-\displaystyle\sum\nolimits_d\durationpdf^{\type_t}_i(d)\valueDPsimple_{i, t + d}
\end{equation}
 \begin{remark}
Later in \Cref{sec:stochastic-infinite}, we will replace this simple dynamic programming with a slightly modified one that has \emph{inventory dependent} state, but is still low dimensional. This allows us to obtain optimal competitive ratios in the setting when rental times are infinite, improving upon the result of \cite{RST-17}.
\end{remark}

\subsubsection{The Final Algorithm}
Inspired by the dynamic programming for the automatic-replenished inventory problem in \Cref{sec:stochastic-finite-simple-DP}, we propose our simulation-based algorithm (\Cref{alg:SB}).
\begin{algorithm}
	\caption{Simulation-based Algorithm with Per-unit Revenue Thresholds }
	\label{alg:SB}
	\begin{algorithmic}[1]
	\vspace{2mm}
	\State{Compute the optimal assignment of $\EAR{\typedistributionsequence}$ given access to the offline assortment oracle  (\Cref{asp:oracle}). Let  $\{\curalloctypeopt\}$ be the optimal assignment.} 
	
	\State{Set $\curexantetype\triangleq\curalloctypeopt\typedistribution_t(\type_t)$ for every $\assortment$,$t$ and $\type_t$ where optimal assignment has a non-zero entry.}	
	\State{Solve the dynamic programming with Bellman update described in \cref{eq:bellman-equation-finite} and boundary condition $\valueDPsimple_{i,T+1}=0$ for every product $i$ to obtain $\{\valueDPsimple_{i,t}\}_{i\in[n],t\in[\totaltime]}$.}
	\State{Let $\curprice\triangleq \valueDPsimple_{i, t + 1}-\displaystyle\sum\nolimits_d\durationpdf_i^{\type_t}(d)\valueDPsimple_{i, t + d}$}, for all $i\in[n],t\in[\totaltime],\type_t\in\typespace_t$.
	\For{time $t=1$ to $T$}
	\State{Realize the consumer type $\type_t\in\typespace_t$.}
	\State {Sample $\hat{\assortment}\sim \{\curalloctypeopt\}_{\assortment\in\assortmentspace}.$}
	\For{products $i\in\hat{\assortment}$}
	\State{Let $I_i$ be the current inventory of product $i$.}
	\State{If $I_i=0$ or $\curreward<\curprice$, remove $i$ from $\hat{\assortment}$.}
	\EndFor
	\State{Offer subset $\hat{\assortment}$ to the current consumer.}
	\EndFor
	\end{algorithmic}
\end{algorithm}

\begin{theorem}
	\label{thm:stochastic-finite-competitive-ratio}
	The competitive ratio of \Cref{alg:SB} against offline Bayesian expected LP benchmark, i.e., $\EAR{\typedistributionsequence}$, is at least $1/2$. Moreover, it runs in time $\textrm{Poly}(n,T, \sum_{t\in[\totaltime]}\lvert\typespace_t\rvert)$ given oracle access to an offline algorithm for assortment optimization (\Cref{asp:oracle}).
\end{theorem}
\subsubsection{Proof of \Cref{thm:stochastic-finite-competitive-ratio}}

The proof of  \Cref{thm:stochastic-finite-competitive-ratio} can be decoupled across products. For each fixed product $i$, we finish the proof in two parts. We first compare \Cref{alg:SB} with the simple dynamic programming described in \Cref{sec:stochastic-finite-simple-DP} and show the total expected revenue of \Cref{alg:SB} due to rentals of product $i$ is at least $\inventory_i\valueDPsimple_{i,1}$ (\texttt{Part~\rom{1}}). We then compare this simple dynamic programming with expected linear programming benchmark and show for each product $i$, $\inventory_i\valueDPsimple_{i,1}$ is at least $1/2$ of the contribution of product $i$ to the optimal objective value of $\EAR{\typedistributionsequence}$ (\texttt{Part~\rom{2}}).
\paragraph{ Proof of \texttt{Part~\rom{1}}.} In this part, we use vector variable $\mathbf{J}=(J_{1},\ldots,J_{T})$ to track the state of inventory of the fixed product $i$, where $J_{t}$ is the number of copies of product $i$ that will return to inventory at time $t$. Note that at each time $t$, a \emph{possible state} $\mathbf{J}$ has the form
\begin{equation*}
\mathbf{J}=(0,\ldots,0,J_{t},J_{t+1},\ldots,J_T)~,
\end{equation*}
where $\sum_{\tau=t}^{T}J_{t}=\inventory_i$. Now suppose $\algValue_{i,t}(\mathbf{J})$ denotes the per-unit revenue of product $i$ generated by \Cref{alg:SB} from time $t$ to $T$, when algorithm starts from initial state $\mathbf{J}$ at time $t$.\footnote{Equivalently, $\algValue_{i,t}(\mathbf{J})$ is equal to the total revenue of product $i$ generated in $[t:T]$ divided by $J_t$,  which is the number of on-hand copies at starting time $t$.} As a convention, let $\algValue_{i,T+1}(\mathbf{J})=0$. We prove the following stronger lemma, which also shows total revenue generated from product $i$ is no less than $\inventory_i\valueDPsimple_{i,1}$.
\begin{lemma} 
\label{lem:part-one-simple}
For every $t\in[\totaltime]$ and every possible inventory state $\mathbf{J}$ at time $t$, $\algValue_{i,t}(\mathbf{J})\geq \valueDPsimple_{i,t}$.
\end{lemma}
\begin{proof} For the base of induction, $\algValue_{i,T+1}(\mathbf{J})=\valueDPsimple_{i,T+1}=0$. Now suppose for any time in $[t+1:T]$ and possible state $\mathbf{J}$ the statement of lemma holds. We can simply write the following update equation for $\algValue_{i,T+1}(\mathbf{J})$ (following exactly the same logic as the update rule of the dynamic programming in \cref{eq:bellman-equation-finite}, but considering that only $J_t$ products are on-hand):
\begin{align}
		\label{eq:bellman-alg}
		\begin{split}
			&\algValue_{i,t}(\mathbf{J})= \displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
		\curexantetype \Bigg(\indicator{\curreward<\curprice}\algValue_{i, t + 1}(\mathbf{J'})+\indicator{\curreward\geq\curprice}\\
& 
		\times\left(\left(1 - \curchoice\right)\algValue_{i, t + 1}(\mathbf{J'}) + \frac{\curchoice}{J_t}\sum\nolimits_d\durationpdf_i^{\type_t}(d)\left(\curreward+\expect{\algValue_{i, t + d}(\mathbf{\tilde{J}^{(d,d)}})+(J_t-1)\algValue_{i, t + 1}(\mathbf{\tilde{J}^{(1,d)}})}\right)\right)\Bigg)
	\end{split}
	\end{align}
where $\mathbf{J'}\triangleq(0,\ldots,0,0,J_t+J_{t+1},J_{t+2},\ldots,J_T)$ is the next state at time $t+1$ if no rental happens at time $t$,  and $\mathbf{\tilde{J}^{(i,d)}}$ is the (randomized) state of \Cref{alg:SB} at time $t+i$ if a rental happens at time $t$ with rental duration $d$ (where the randomness in this state comes from all type realizations and consumer choices during future times $[t+1:t+d-1]$). Now, By applying our inductive hypotheses to \cref{eq:bellman-alg}, we have: 
\begin{align*}
		\begin{split}
			&\algValue_{i,t}(\mathbf{J})\geq \displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
		\curexantetype \Bigg(\indicator{\curreward<\curprice}\valueDPsimple_{i,t+1}+\\
& 
		+\indicator{\curreward\geq\curprice}\left(\left(1 - \curchoice\right)\valueDPsimple_{i,t+1} + \frac{\curchoice}{J_t}\sum\nolimits_d\durationpdf_i^{\type_t}(d)\left(\curreward+\valueDPsimple_{i,t+d}+(J_t-1)\valueDPsimple_{i,t+1}\right)\right)\Bigg)
	\end{split}
	\end{align*}
Note also that the RHS of above inequality is non-increasing as a function of $J_t$, simply because if $\frac{1}{J_t}$  increases by additive $\epsilon>0$ then RHS increases by 
\begin{align*}
&\epsilon\cdot\indicator{\curreward\geq\curprice}\cdot \curchoice\cdot\left(\sum\nolimits_d\durationpdf_i^{\type_t}(d)(\curreward+\valueDPsimple_{i,t+d}-\valueDPsimple_{i,t+1})\right)\\
=&\epsilon\cdot\indicator{\curreward\geq\curprice}\cdot \curchoice\cdot\left(\curreward-\curprice\right)\geq 0
\end{align*}
Therefore, as $J_t\leq \inventory_i$, we have
\begin{align*}
		\begin{split}
			\algValue_{i,t}(\mathbf{J})&\geq \displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
		\curexantetype \Bigg(\indicator{\curreward<\curprice}\valueDPsimple_{i,t+1}+\\
& 
		+\indicator{\curreward\geq\curprice}\left(\left(1 - \curchoice\right)\valueDPsimple_{i,t+1} + \frac{\curchoice}{\inventory_i}\sum\nolimits_d\durationpdf_i^{\type_t}(d)\left(\curreward+\valueDPsimple_{i,t+d}+(\inventory_i-1)\valueDPsimple_{i,t+1}\right)\right)\Bigg)\\
		&=\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
		\curexantetype \\
& 
		\times\max\left\{\valueDPsimple_{i, t + 1}~,~\left(1 - \curchoice\right)\valueDPsimple_{i, t + 1}+ \curchoice\left(\frac{1}{\inventory_i}\sum\nolimits_d\durationpdf_i^{\type_t}(d)\left(\curreward+\valueDPsimple_{i, t + d}\right)+\frac{\inventory_i-1}{\inventory_i}\valueDPsimple_{i, t + 1}\right )\right\}\\
		&=\valueDPsimple_{i, t }\qquad\qquad\qquad\qquad\qquad\qquad \textrm{(holds because of Bellman update in \cref{eq:bellman-equation-finite})}
	\end{split}
	\end{align*}
\end{proof}

\paragraph{ Proof of \texttt{Part~\rom{2}}.} In order to prove this part, we use the connection between DP of \Cref{sec:stochastic-finite-simple-DP} and a related LP. This connections leads us to apply simple dulaity arguments to find a lower-bound on the ratio of $\inventory_i\valueDPsimple_{i,1}$ and the contribution of product $i$ to the optimal objective value of $\EAR{\typedistributionsequence}$. Similar techniques have also been proposed in \cite{DA-09,A-07}, and also in \cite{AHL-12,ala-14} for other problems .

Note that scaling $\{\curreward\}$  does not change the ratio. Hence, w.l.o.g. we can assume:
\begin{equation*}
\displaystyle\sum\nolimits_{t=1}^{\totaltime}
			\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
			\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}\curexantetype\curchoice
			\curreward
			 =1
\end{equation*}
Given the above observation and the Bellman update in \cref{eq:bellman-equation-finite}, consider the following primal linear program that gives a lower-bound on worst-case value of the ratio:
\begin{align}
		\begin{array}{llll}
			{\min
			\limits_{\mathbf \reward, \boldsymbol\valueDPsimple \geq \mathbf 0}}~~&
				\inventory_i\valueDPsimple_{i,1}~~~\text{s.t.}& \\[1em]
							&
			\valueDPsimple_{i,t}\geq	\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
		\curexantetype~~~~~~~~~~~~~~~~~~~~~~~~~~\forall t \\
& 
		\times\max\left\{\valueDPsimple_{i, t + 1}~,~\left(1 - \curchoice\right)\valueDPsimple_{i, t + 1}+ \curchoice\left(\frac{1}{\inventory_i}\sum\nolimits_d\durationpdf_i^{\type_t}(d)\left(\curreward+\valueDPsimple_{i, t + d}\right)+\frac{\inventory_i-1}{\inventory_i}\valueDPsimple_{i, t + 1}\right )\right\}
			\\[1em]
			&
			\displaystyle\sum\nolimits_{t=1}^{\totaltime}
			\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
			\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
			\curexantetype\curchoice
			\curreward
			\geq1& &
		\end{array}
	\end{align}
in which we allow both $\boldsymbol{\valueDPsimple}=\{\valueDPsimple_{i,t}\}_{t=1}^T$ and $\mathbf{\reward}=\{\curreward\}_{t\in[\totaltime],\type_t\in\typespace_t}$ to be variables (and this is an important feature of this technique). We first relax and simplify this program by switching the outer summation and max operator in the RHS of the first constraint (which only makes RHS smaller, hence a relaxation). Note also that:
\begin{align*}
&\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}\curexantetype\valueDPsimple_{i, t + 1}=\valueDPsimple_{i, t + 1}\triangleq A,\\
&\textrm{and}\\
	&\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}\curexantetype\left(\left(1 - \curchoice\right)\valueDPsimple_{i, t + 1}+ \curchoice\left(\frac{1}{\inventory_i}\sum\nolimits_d\durationpdf_i^{\type_t}(d)\left(\curreward+\valueDPsimple_{i, t + d}\right)+\frac{\inventory_i-1}{\inventory_i}\valueDPsimple_{i, t + 1}\right )\right)	\\
		&=\frac{1}{\inventory_i}\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
		\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}\curexantetype\curchoice\left(\sum\nolimits_d\durationpdf_i^{\type_t}(d)\left(\curreward+\valueDPsimple_{i, t + d}\right)-\valueDPsimple_{i, t + 1}\right)+\valueDPsimple_{i, t + 1}\triangleq B
\end{align*}
Now, by replacing the new constraint $\valueDPsimple_{i, t}\geq \max\{A,B\}$ with two constraints $\valueDPsimple_{i, t}\geq A$ and $\valueDPsimple_{i, t}\geq B$,  we get the following final primal linear programming:
\begin{align}
\label{eq:stochastic-finite-primal}\tag{\textbf{Primal-LP1}}
		\begin{array}{llll}
			{\min
			\limits_{\mathbf \reward, \boldsymbol\valueDPsimple \geq \mathbf 0}}~~&
				\inventory_i\valueDPsimple_{i,1}~~~~~\text{s.t.}& & \\[1em]
			&\valueDPsimple_{i,t}\geq	\frac{1}{\inventory_i}\displaystyle\sum\nolimits_{\type_t \in \typespace_t,\assortment \in \assortmentspace}
		\curexantetype\curchoice\left(\sum\nolimits_d\durationpdf_i^{\type_t}(d)\left(\curreward+\valueDPsimple_{i, t + d}\right)-\valueDPsimple_{i, t + 1}\right)+\valueDPsimple_{i, t + 1} & t\in[\totaltime]&\langle\alpha_t\rangle\\[1em] 
		&\valueDPsimple_{i,t}\geq	\valueDPsimple_{i,t+1}&t\in[\totaltime] &\langle\beta_t\rangle\\[1em]
			&\displaystyle\sum\nolimits_{t=1}^{\totaltime}
			\displaystyle\sum\nolimits_{\type_t \in \typespace_t}
			\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
			\curexantetype\curchoice
			\curreward
			\geq1& &\langle\mu \rangle
		\end{array}
	\end{align}
 Now, we write its dual program with dual variable $\{\alpha_t\}$, $\{\beta_t\}$ and $\mu$ as follows:

\begin{align}
\label{eq:stochastic-finite-dual}\tag{\textbf{Dual-LP1}}
		\begin{array}{llll}
			&{\max\limits_{\boldsymbol\alpha, \boldsymbol\beta, \mu\geq \mathbf 0}}~~
				\mu~~~~~\text{s.t.}& &\\[1em]
				&\mu\left(\displaystyle\sum\nolimits_{t=1}^{\totaltime}
			\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
			\curchoice
			\curexantetype\right)\leq \frac{1}{\inventory_i}\left(\displaystyle\sum\nolimits_{t=1}^{\totaltime}
			\displaystyle\sum\nolimits_{\assortment \in \assortmentspace}
			\curchoice
			\curexantetype\alpha_t\right)& \type_t\in\typespace_t &\langle\curreward \rangle\\[1em]
			&\alpha_t-\alpha_{t-1}+\beta_t-\beta_{t-1}\leq \frac{1}{\inventory_i} \displaystyle\sum\nolimits_{\type_{t-1} \in \typespace_{t-1},\assortment \in \assortmentspace}X_{S,t-1,\type_{t-1}}\choice^{\type_{t-1}}(S,i)\alpha_{t-1} & &\\
			&\qquad\qquad\qquad\qquad\qquad -\frac{1}{\inventory_i} \displaystyle\sum\nolimits_{d< t}   \displaystyle\sum\nolimits_{\type_{t-d} \in \typespace_{t-d},\assortment \in \assortmentspace}g_i^{\type_{t-d}}X_{S,t-d,\type_{t-d}}\choice^{\type_{t-d}}(S,i)\alpha_{t-d} & t\in[2:T] & \langle\valueDPsimple_{i,2:T} \rangle\\[1em]
			&\alpha_1+\beta_1\leq \inventory_i& & \langle\valueDPsimple_{i,1} \rangle
		\end{array}
\end{align}
Now, we try to guess a feasible solution for the dual program to obtain our desired lower-bound on the optimal primal objective. To this end, let $\forall t: \alpha_t=\mu\inventory_i$ (therefore, first set of constraints will be satisfied automatically) and let all other constraints to be tight. In particular, $\beta_1=\inventory_i-\alpha_1=\inventory_i(1-\mu)$ and for all $t\in [2:T]$:
\begin{align*}
\beta_t&=\beta_{t-1}+\frac{1}{\inventory_i} \displaystyle\sum\nolimits_{\type_{t-1} \in \typespace_{t-1},\assortment \in \assortmentspace}X_{S,t-1,\type_{t-1}}\choice^{\type_{t-1}}(S,i)\alpha_{t-1} &\\
			 &\qquad\quad-\frac{1}{\inventory_i} \displaystyle\sum\nolimits_{d< t}   \displaystyle\sum\nolimits_{\type_{t-d} \in \typespace_{t-d},\assortment \in \assortmentspace}g_i^{\type_{t-d}}X_{S,t-d,\type_{t-d}}\choice^{\type_{t-d}}(S,i)\alpha_{t-d} & \\
			&=\beta_{t-1}+\mu \displaystyle\sum\nolimits_{\type \in \typespace_{t-1},\assortment \in \assortmentspace}X_{S,t-1,\type}\choice^{\type}(S,i)&\\
			 &\qquad\quad-\mu\displaystyle\sum\nolimits_{d< t}   \displaystyle\sum\nolimits_{\type\in \typespace_{t-d},\assortment \in \assortmentspace}g_i^{\type}X_{S,t-d,\type}\choice^{\type}(S,i)& \\
			 &\overset{(1)}{=}\beta_1-\mu \displaystyle\sum\nolimits_{\tpre\leq t}\displaystyle\sum\nolimits_{\type \in \typespace_{t},\assortment \in \assortmentspace}X_{S,\tpre,\type}\choice^{\type}(S,i)\sum_{d\geq t-\tpre}\durationpdf_i^{\type}(d)&\\
			 &\overset{(2)}{\geq }\inventory_i(1-\mu)-\mu\inventory_i=\inventory_i(1-2\mu)~,
\end{align*}
where (1) can be obtained by changing the order of summations and rearranging the terms, and (2) holds because of inventory feasibility of $\{\curalloctypeopt\}$ in expectation in $\EAR{\typedistributionsequence}$. Now, setting $\mu=1/2$ guarantees dual feasibility as $\forall t: \alpha_t\geq 0,\beta_t\geq 0$, and other constraints of the dual are satisfied by construction. By applying weak duality, the desired ratio is at least $\mu=1/2$, which finishes the proof.





\subsection{Improved Simulation-based Algorithms for Infinite Rental Times}
\label{sec:stochastic-infinite}
\input{tex/stochastic-no-duration.tex}

\subsection{Discussion on Advanced Reservation}
\label{sec:stochastic-duration-revealed}
\input{tex/stochastic-exact-duration.tex}


